Asymptotic convergence rates for coordinate descent in polyhedral sets

We consider a family of parallel methods for constrained optimization based on projected gradient descents along individual coordinate directions. In the case of polyhedral feasible sets, local convergence towards a regular solution occurs unconstrained in a reduced space, allowing for the computation of tight asymptotic convergence rates by sensitivity analysis, this even when global convergence rates are unavailable or too conservative. We derive linear asymptotic rates of convergence in polyhedra for variants of the coordinate descent approach, including cyclic, synchronous, and random modes of implementation. Our results find application in stochastic optimization, and with recently proposed optimization algorithms based on Taylor approximations of the Newton step.

==> tubmacros.tex <==
\newcommand{\llamb}{y}
\newcommand{\deltalamb}{z}
\newcommand{\freexx}{\tilde \xx}
\newcommand{\mmu}{z}
\newcommand{\lambdaset}{Y}
\newcommand{\nn}{n}
\newcommand{\ee}{l}
\newcommand{\NN}{N}
\newcommand{\MM}{M}
\newcommand{\setofnodes}{V}
\newcommand{\setofneighbours}{\mathcal{N}}
%\newcommand{\setoflambdasol}{\bar\lambdaset}
%\newcommand{\genericset}{\Omega}
%\newcommand{\genericsettwo}{Y}
%\newcommand{\hood}{X}
%\newcommand{\Scale}{S}
%\newcommand{\diagScale}{D}
%\newcommand{\mapping}{\mathbf{P}}
%\newcommand{\Smapping}{\mathbf{S}}
%\newcommand{\Amapping}{\mathbf{A}}
%\newcommand{\alphamapping}{\alpha}
%\newcommand{\newtonmapping}{\mathbf{N}}
%\newcommand{\newtonmapping}{\mathbf{N}}
%\newcommand{\Zmapping}{\mathbf{Z}}
%\newcommand{\mapfunction}{\mathcal{M}}
%\newcommand{\mapGfunction}{\mathcal{G}}
%\newcommand{\mapAfunction}{a}
%\newcommand{\mapSfunction}{\mathcal{S}}
%\newcommand{\mapOfunction}{\mathcal{O}}
%\newcommand{\sequencesymbol}{\gamma}
%\newcommand{\yyk}[1]{\mu^{#1}}
%\newcommand{\buff}{z}
\newcommand{\llambother}{z}
\newcommand{\LCmu}{\tilde z}
%\newcommand{\mapx}{x}
%\newcommand{\mapX}{X}
%\newcommand{\proj}[1]{P^{#1}}
%\newcommand{\projT}[2]{P^{#1}}
%\newcommand{\projx}[2]{P^{#1}({#2})}
%\newcommand{\projTx}[3]{P^{#1}({#3};{#2})}
%\newcommand{\vect}[1]{\text{vect}({#1})}
%\newcommand{\Vect}[1]{\left({#1}\right)}
%\newcommand{\linevect}[1]{({#1})}
%\newcommand{\notx}{x}
%\newcommand{\notv}{v}
%\newcommand{\notvi}[1]{\notv_{#1}}
%\newcommand{\llambconvij}[2]{\llambconv_{{#1},{#2}}}
%\newcommand{\llambij}[2]{\llamb_{{#1},{#2}}}
%\newcommand{\noty}{y}
%\newcommand{\notz}{z}
%\newcommand{\notf}{f}
%\newcommand{\notg}{g}
%\newcommand{\notF}{F}
%\newcommand{\CCLone}{\mathcal{F}}
%\newcommand{\stoch}{\omega}
%\newcommand{\Stoch}{\Omega}
%\newcommand{\stochFfunction}{F}
%\newcommand{\stochxfunction}{x}
%\newcommand{\stochXfunction}{{X}}
%\newcommand{\functionalX}{\mathcal{X}}
%\newcommand{\stochobjectivefunction}{\objectivefunction}
%\renewcommand{\function}{f} 
%\newcommand{\setoffunctions}{\mathcal{F}}
%\newcommand{\stochdualfunction}{\bar\dualfunction}
%\newcommand{\stochlagrangianfunction}{\bar l}
%\newcommand{\stochlfunction}{l}
%\newcommand{\stochgfunction}{\dualfunction}
%\newcommand{\sd}{s}
\newcommand{\genericnormscale}{\Scale}
\newcommand{\violatingsymbol}{E}
\newcommand{\orderingsymbol}{O}
\newcommand{\violatingsetsymbol}{\mathcal{I}}
\newcommand{\identitysymbol}{I}
\newcommand{\matrixidentitysymbol}{W}
%\newcommand{\constraintfunction}{c}
%\newcommand{\constraintlocalijfunction}[2]{\varsigma_{{#1}{#2}}}
%\newcommand{\cconst}{\varsigma}
%\newcommand{\constraintineqlocalconst}{p}
%\newcommand{\directedgraph}{\mathcal{G}}
%\newcommand{\bvector}{b}
%\newcommand{\incidence}{A}
%\newcommand{\setofedges}{E}
%\newcommand{\positive}[1]{({#1})^{+}}
%\newcommand{\nonPROJx}{x}
\newcommand{\grad}{\nabla} %\newcommand{\grad}{\boldsymbol{\nabla}}
\newcommand{\gradient}[1]{\grad_{\!{#1}}}
\newcommand{\gradij}[2]{\grad_{\! {#1},{#2}}}
\newcommand{\gradfxij}[3]{\gradfij{#2}{#3} ( {#1} )}
\newcommand{\gradfx}[1]{\gradf ( {#1} )}
\newcommand{\gradi}[1]{\grad_{\! #1}}
\newcommand{\gradf}{\grad \dualfunction}
\newcommand{\gradfi}[1]{\gradi{#1}\dualfunction}
\newcommand{\gradfxi}[2]{\gradfi{#2} ( {#1} )}
\newcommand{\gradfij}[2]{\gradij{#1}{#2}\dualfunction}
\newcommand{\jacobianfunction}[1]{{J}{#1}} %\newcommand{\jacobianfunction}[1]{J({#1})}
\newcommand{\jacobianifunction}[2]{\jacobianfunction{#1}_{#2}}
\newcommand{\jacobianijfunction}[3]{\jacobianfunction{#1}_{{#2}{#3}}}
\newcommand{\hessianfunction}[1]{\nabla^2{#1}}
\newcommand{\hessiantildefunction}[1]{\tilde\nabla^2{#1}}
\newcommand{\hessianifunction}[2]{\nabla^2_{\! {#2}}{#1}}
\newcommand{\hessiantildeifunction}[2]{\tilde\nabla^2_{\! {#2}}{#1}}
\newcommand{\HYBrho}{\psi}%{\rho}
\newcommand{\HYBRho}{\Psi}
\newcommand{\setst}{\, | \,}
\newcommand{\REALplusone}{\REALone_{\geq 0\!}}%{\REALone_{\text{\tiny{\ensuremath{\geq 0}}}}}%{\REALone^{\!\text{\textup{\tiny{+}}}}}
\newcommand{\REALpluszeroone}{\REALone_{> 0\!}}%{\REALone^{\!\text{\textup{\tiny{+}}}}}%{\REALone_{0}^{\!\text{\textup{\tiny{+}}}}}
\newcommand{\REALplus}[1]{\REALone_{\geq 0\!}^{#1}}%{\REALone^{\!{\text{\textup{\tiny{+}}}}{#1}}}


%\newcommand{\llamb}{\lambda}
%\newcommand{\deltalamb}{\gamma}
%\newcommand{\freexx}{\yy}
%\newcommand{\mmu}{\mu}
%\newcommand{\lambdaset}{\Lambda}
%\newcommand{\nn}{n}
%\newcommand{\ee}{p}
%\newcommand{\NN}{N}
%\newcommand{\MM}{M}
%\newcommand{\setofnodes}{V}
%\newcommand{\setofneighbours}{\mathcal{N}}
\newcommand{\setoflambdasol}{\tilde\lambdaset}
\newcommand{\genericset}{X}
\newcommand{\genericsettwo}{Y}
\newcommand{\hood}{\Omega}
\newcommand{\Scale}{T}
\newcommand{\diagScale}{D}
\newcommand{\mapping}{\mathbf{G}}
\newcommand{\Smapping}{\mathbf{S}}
\newcommand{\Amapping}{\mathbf{A}}
\newcommand{\alphamapping}{\alpha}
\newcommand{\newtonmapping}{\mathbf{N}}
\newcommand{\Zmapping}{\mathbf{N}} %{\mathbf{Z}}
\newcommand{\mapfunction}{\mathcal{M}}
\newcommand{\mapGfunction}{\mathcal{G}}
\newcommand{\mapAfunction}{a}
\newcommand{\mapSfunction}{\mathcal{S}}
\newcommand{\mapOfunction}{\mathcal{O}}
\newcommand{\mapGGfunction}{\mathcal{H}}
\newcommand{\sequencesymbol}{x}
\newcommand{\yyk}[1]{z^{#1}}
\newcommand{\buff}{z}
%\newcommand{\llambother}{\mu}
%\newcommand{\LCmu}{\tilde \mu}
\newcommand{\mapx}{x}
\newcommand{\mapX}{X}
\newcommand{\proj}[1]{\left\lbrack . \right\rbrack^{+}_{{#1}}}
\newcommand{\projT}[2]{\left\lbrack . \right\rbrack^{+}_{{#1},{#2}}}
\newcommand{\projx}[2]{\left\lbrack {#2} \right\rbrack^{+}_{{#1}}}
\newcommand{\projTx}[3]{\left\lbrack {#3} \right\rbrack^{+}_{{#1},{#2}}}
\newcommand{\vect}[1]{({#1})}
\newcommand{\Vect}[1]{\left({#1}\right)}
\newcommand{\linevect}[1]{({#1})}
\newcommand{\lvs}{\ \,}
\newcommand{\notx}{x}
\newcommand{\notv}{v}
\newcommand{\notvi}[1]{\notv_{#1}}
\newcommand{\llambconvij}[2]{(\llambconv_{#1})_{#2}}
\newcommand{\llambij}[2]{(\llamb_{#1})_{#2}}
\newcommand{\noty}{y}
\newcommand{\notz}{z}
\newcommand{\notf}{f}
\newcommand{\notg}{g}
\newcommand{\notF}{F}
\newcommand{\CCLone}{G} %{\mathcal{G}}
\newcommand{\stoch}{\omega}
\newcommand{\stochtwo}{\nu}%{\varpi}
\newcommand{\Stoch}{\Omega}
\newcommand{\stochFfunction}{F}
\newcommand{\stochxfunction}{x}
\newcommand{\stochXfunction}{{X}}
\newcommand{\functionalX}{\mathcal{X}}
\newcommand{\stochobjectivefunction}{\objectivefunction}
\renewcommand{\function}{\dualfunction} 
\newcommand{\stochdualfunction}{\function}
\newcommand{\stochlagrangianfunction}{l}
\newcommand{\stochlfunction}{\tilde l}
\newcommand{\stochgfunction}{\tilde \function}
\newcommand{\sd}{\bar s}
%\newcommand{\genericnormscale}{G}
%\newcommand{\violatingsymbol}{E}
%\newcommand{\orderingsymbol}{O}
%\newcommand{\violatingsetsymbol}{I}
%\newcommand{\identitysymbol}{I}
%\newcommand{\matrixidentitysymbol}{W}
\newcommand{\constraintfunction}{c}
\newcommand{\constraintlocalijfunction}[2]{\varsigma_{{#1}{#2}}}
\newcommand{\cconst}{\varsigma}
\newcommand{\constraintineqlocalconst}{d}
\newcommand{\directedgraph}{\mathcal{G}}
\newcommand{\bvector}{b}
\newcommand{\incidence}{A}
\newcommand{\setofedges}{E}
\newcommand{\positive}[1]{({#1})^{+}}
\newcommand{\nonPROJx}{x}
%\newcommand{\gradient}[1]{\nabla_{\!{#1}}}
%\newcommand{\grad}{\nabla}
%\newcommand{\gradij}[2]{\nabla_{\! {#1},{#2}}}
%\newcommand{\gradfxij}[3]{(\gradfxi{#1}{#2})_{#3}}
%\newcommand{\gradfx}[1]{\gradf ( {#1} )}
%\newcommand{\gradi}[1]{\grad_{\! #1}}
%\newcommand{\gradf}{\grad \dualfunction}
%\newcommand{\gradfi}[1]{\gradi{#1}\dualfunction}
%\newcommand{\gradfxi}[2]{\gradfi{#2} ( {#1} )}
%\newcommand{\gradfij}[2]{\gradij{#1}{#2}\dualfunction}
%\newcommand{\jacobianfunction}[1]{J({#1})}
%\newcommand{\jacobianifunction}[2]{\jacobianfunction{#1}_{#2}}
%\newcommand{\jacobianijfunction}[3]{\jacobianfunction{#1}_{{#2}{#3}}}
%\newcommand{\hessianfunction}[1]{H^{#1}}
%\newcommand{\hessiantildefunction}[1]{\tilde H^{#1}}
%\newcommand{\hessianifunction}[2]{\hessianfunction{#1}_{#2}}
%\newcommand{\hessiantildeifunction}[2]{\hessiantildefunction{#1}_{#2}}
%\newcommand{\HYBrho}{\psi}%{\rho}
%\newcommand{\HYBRho}{\Psi}
%\newcommand{\setst}{:}
%\newcommand{\REALplusone}{\REALone^{\!\text{\textup{\tiny{+}}}}}
%\newcommand{\REALpluszeroone}{\REALone_{0}^{\!\text{\textup{\tiny{+}}}}}
%\newcommand{\REALplus}[1]{\REALone^{\!{\text{\textup{\tiny{+}}}}{#1}}}



%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\limsup}[1]{\lim_{#1} \sup}
%%\newcommand{\liminf}[1]{\lim_{#1} \inf}


\newcommand{\loga}[1]{\log_{#1}}
\newcommand{\logn}{\ln}%{\log}

%%%

\newcommand{\llambi}[1]{\llamb_{#1}}
\newcommand{\llambconv}{\llamb^\star}
\newcommand{\llambconvi}[1]{\llambconv_{#1}}
\newcommand{\mmui}[1]{\mmu_{#1}}
\newcommand{\llambcs}{\llamb^*}
\newcommand{\llambcsi}[1]{\llambcs_{#1}}
\newcommand{\lambdaone}{\llamb}
\newcommand{\lambdatwo}{\mmu}
\newcommand{\xx}{x}
\newcommand{\XX}{X}
\newcommand{\xxi}[1]{\xx_{#1}}
\newcommand{\tildexx}{\tilde \xx}
\newcommand{\tildexxi}[1]{\tildexx_{#1}}
\newcommand{\xxsol}{\xx^\star}
\newcommand{\XXoptfunction}{\Xsolfunction}
\newcommand{\XXopt}[1]{\XXoptfunction({#1})}
\newcommand{\xxoptfunction}{\xsolfunction}
\newcommand{\xxopt}[1]{\xxoptfunction({#1})}
\newcommand{\xxoptifunction}[1]{\xxoptfunction_{#1}}
\newcommand{\xxopti}[2]{\xxoptifunction{#1}({#2})}

%\newcommand{\xxprime}{x^{\prime}}
%\newcommand{\xxprimei}[1]{\xxprime_{#1}}
\newcommand{\xbar}{\bar x}
\newcommand{\xbari}[1]{\xbar_{#1}}
\newcommand{\xtilde}{\tilde x}
\newcommand{\xtildei}[1]{\xtilde_{#1}}
\newcommand{\xk}[1]{x_{#1}}
\newcommand{\xki}[2]{x_{#1}^{#2}}
\newcommand{\NNi}[1]{\NN_{#1}}
\newcommand{\Qset}{X}
\newcommand{\Qseti}[1]{\Qset_{#1}}
\newcommand{\mm}{m}
%\newcommand{\MMeq}{\MM^{\text{e}}}
%\newcommand{\MMineq}{\MM^{\text{i}}}
\newcommand{\MMeq}{u}
\newcommand{\MMineq}{v}
\newcommand{\MMi}[1]{\MM_{#1}}
\newcommand{\MMeqi}[1]{\MMeq_{#1}}
\newcommand{\MMineqi}[1]{\MMineq_{#1}}
\newcommand{\tildeMM}{\tilde \MM}
\newcommand{\tildeMMi}[1]{\tildeMM_{#1}}
\newcommand{\setoflambdas}{\lambdaset}
\newcommand{\setoflambdasi}[1]{\setoflambdas_{#1}}
\newcommand{\setoflambdasolk}[1]{\setoflambdasol^{#1}}
\newcommand{\fni}{\varrho}
\newcommand{\setofnnc}{\mathcal{P}}
\newcommand{\setofnnci}[1]{\setofnnc_{#1}}
\newcommand{\setofuc}{\mathcal{U}}
\newcommand{\setofuci}[1]{\setofuc_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\wpone}{w.p.$1${}}

%%
\newcommand{\distance}[2]{\textnormal{dist}({#1},{#2})}

\newcommand{\notfx}[1]{\notf({#1})}
\newcommand{\Notfx}[1]{\notf\left({#1}\right)}
\newcommand{\notgx}[1]{\notg({#1})}
\newcommand{\notfk}[1]{\notf^{#1}}
\newcommand{\notfkx}[2]{\notfk{#1}({#2})}
\newcommand{\notfi}[1]{\notf_{#1}}
\newcommand{\notfix}[2]{\notfi{#1}({#2})}

\newcommand{\spectralradiusfunction}{\rho}
\newcommand{\spectralradius}[1]{\spectralradiusfunction({#1})}
\newcommand{\Spectralradius}[1]{\spectralradiusfunction\left({#1}\right)}




\newcommand{\nbpi}{t_0}
\newcommand{\nbpiprime}{t}
%\newcommand{\nbliberty}{\nbpiprime^\prime}
%\newcommand{\nblibertyi}[1]{\nbliberty_{#1}}

\newcommand{\intersection}[1]{{\cap}_{#1}}
\newcommand{\argmin}[1]{\arg \, \min_{#1}\,}
%\newcommand{\argmax}[1]{\arg \ \max_{#1}}

\newcommand{\functionstart}[1]{#1\\ \hline}
\newcommand{\functionending}{\\ \hline}
\newcommand{\newentry}{\ -\ }
\newcommand{\newblankentry}{\ \ \ }
\newcommand{\onetab}{\ \ \, }
\newcommand{\twotabs}{\onetab \onetab}
\newcommand{\threetabs}{\twotabs \onetab}
\newcommand{\fourtabs}{\threetabs \onetab}

%\newcommand{\minimise}[1]{\underset{#1}{\text{minimise}}}
%\newcommand{\function}{f} % conflict with package {algorithm2e}
\newcommand{\fx}[1]{\function ({#1})}
\newcommand{\fxi}[2]{\function_{#2} ({#1})}
%\newcommand{\gradfi}[1]{\gradf_{#1}}
%\newcommand{\gradfxi}[2]{\gradf_{#2} ( {#1} )}
\newcommand{\functioni}[1]{\function_{#1}}
\newcommand{\functionix}[2]{\function_{#1}({#2})}

%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\diag}[1]{\textup{diag}({#1})}
\newcommand{\bigdiag}[1]{\text{diag}\left({#1}\right)}
\newcommand{\orthogonalprojectionfunction}[1]{P^{#1}}
\newcommand{\orthogonalprojection}[2]{\orthogonalprojectionfunction{#1}({#2})}
\newcommand{\subgradientstep}{a}
\newcommand{\subgradientstepk}[1]{\subgradientstep^{#1}}
\newcommand{\sumin}[2]{\sum_{{#1}=1}^{#2}}

%\newcommand{\REAL}{R}
\newcommand{\RNN}{\REALone^\NN}
\newcommand{\RNNi}[1]{\REALone^{\NN_{#1}}}
\newcommand{\RMM}{\REALone^\MM}
\newcommand{\RMMi}[1]{\REALone^{\MM_{#1}}}
\newcommand{\tildeRMM}{\REALone^\tildeMM}
\newcommand{\tildeRMMi}[1]{\REALone^{\tildeMM_{#1}}}
\newcommand{\Rnn}{\REALone^\nn}



%\newcommand{\xxa}[3]{\xi^{#1} ({#2},{#3})}
%\newcommand{\xxai}[4]{\xi^{#1}_{#4} ({#2},{#3})}
%\newcommand{\iofkj}[2]{i^{#1}({#2})}
\newcommand{\xxafunction}{\xi}
\newcommand{\xxafunctioni}[1]{\xi_{#1}}
\newcommand{\xxa}[3]{\xxafunction ({#2},{#3})}
\newcommand{\xxai}[4]{\xxafunction_{#4} ({#2},{#3})}
\newcommand{\iofkj}[2]{{#2}}

%\newcommand{\aam}[1]{\alpha ({#1})}
%\newcommand{\aami}[2]{\alpha_{#2} ({#1})}
%\newcommand{\aajy}[2]{\alpha({#1};{#2})}
\newcommand{\aafunction}{\alpha}
\newcommand{\aaiTy}[3]{\aafunction({#1},{#2};{#3})}
%\newcommand{\aapdjy}[3]{\alpha^{#1}({#2};{#3})}
\newcommand{\primalalgo}{p}
\newcommand{\dualalgo}{d}

\newcommand{\meanllamb}{\bar\llamb}
\newcommand{\meanllambk}[1]{\meanllamb^{#1}}
\newcommand{\meanllambki}[2]{\meanllamb^{#1}_{#2}}

\newcommand{\llambk}[1]{\llamb^{#1}}
\newcommand{\llambki}[2]{\llamb^{#1}_{#2}}
\newcommand{\llambka}[2]{\llambk{#1} ({#2})}
\newcommand{\llambkai}[3]{\llambki{#1}{#3} ({#2})}
\newcommand{\mmuk}[1]{\mmu^{#1}}
\newcommand{\Pa}{a}
\newcommand{\Pai}[1]{\Pa({#1})}
\newcommand{\Pak}[1]{\Pa^{#1}}
\newcommand{\Paki}[2]{\Pak{#1}({#2})}
\newcommand{\Pm}{m}
\newcommand{\Pmi}[1]{\Pm}%{\Pm_{#1}}
\newcommand{\Pmk}[1]{\Pm^{#1}}
\newcommand{\Pmki}[2]{\Pmk{#1}_{#2}}
\newcommand{\Psig}{\sigma}
\newcommand{\Ps}{s}
\newcommand{\Psnew}{s}
%%\newcommand{\Pssi}[1]{\Ps_{#1}}
%\newcommand{\Pssi}[1]{\Ps}%
%\newcommand{\noPs}[1]{{#1}}
%\newcommand{\changePs}[2]{{#2}}
\newcommand{\Pssi}[1]{}%
\newcommand{\noPs}[1]{}
\newcommand{\changePs}[2]{{#1}}
\newcommand{\Pssmax}{\bar \Ps}
\newcommand{\Pbeta}{\beta}
\newcommand{\Scaletwo}{\hat\Scale}
\newcommand{\Scalei}[1]{\Scale_{#1}}
\newcommand{\Scalek}[1]{\Scale^{#1}}
\newcommand{\Scaleki}[2]{{\Scalek{#1}({#2})}}
\newcommand{\Scalex}[1]{\Scale({#1})}
\newcommand{\Scaleix}[2]{\Scalei{#1}({#2})}
\newcommand{\Scalefx}[2]{\Scale({#1},{#2})}
\newcommand{\Scaleifx}[3]{\Scalei{#1}({#2},{#3})}
\newcommand{\DScale}{\Delta}
\newcommand{\DScalei}[1]{\DScale_{#1}}
\newcommand{\DScaleix}[2]{\DScalei{#1}({#2})}
\newcommand{\DtildeScale}{\tilde\DScale}
\newcommand{\DtildeScalei}[1]{\DtildeScale_{#1}}
\newcommand{\DtildeScaleix}[2]{\DtildeScalei{#1}({#2})}
\newcommand{\eigenTmax}{\eigenTbound}
%\newcommand{\eigenTmax}{\lambda^{max}}
\newcommand{\eigenTmin}{\lambda^{min}}
\newcommand{\eigenTmaxi}[1]{\eigenTmax_{#1}}
\newcommand{\eigenTmini}[1]{\eigenTmin_{#1}}
\newcommand{\eigentbound}{\textup{\b{$\lambda$}}} %{\underline{\lambda}} %{\text{\b{$\lambda$}}}
\newcommand{\eigenTbound}{\bar\lambda} %{\overline{\lambda}} %{\bar\lambda}
%\newcommand{\llambt}[5]{\zeta({#1},{#3},{#4};{#2},{#5})}
\newcommand{\llambt}[5]{\zeta({#5})}
\newcommand{\descentfunction}{\pi}
\newcommand{\descent}[4]{\descentfunction_{#1}({#2};{#3},{#4})}
\newcommand{\Descentfunction}{\hat \descentfunction}
\newcommand{\Descentifunction}[1]{\Descentfunction_{#1}}
\newcommand{\Descent}[4]{\Descentfunction_{#1}({#2};{#3},{#4})}
%\newcommand{\Descentfunction}{p}
%\newcommand{\Descent}[4]{\Descentfunction({#1},{#3},{#4};{#2})}
\newcommand{\Descenti}[5]{\Descentfunction_{#5}({#1},{#3},{#4};{#2})} % obsolete
%\newcommand{\descentfunction}{\pi}
%\newcommand{\descent}[4]{\descentfunction({#1},{#3},{#4};{#2})}
%\newcommand{\descentblank}[1]{\descent{#1}{.}{.}{.}}
\newcommand{\newtonDescentfunction}{n}
\newcommand{\newtonDescent}[2]{\newtonDescentfunction({#1};{#2})}
\newcommand{\newtonDescenti}[3]{\newtonDescentfunction_{#3}({#1};{#2})}
\newcommand{\newtonDescentblank}[1]{\newtonDescent{#1}{.}}
\newcommand{\newtondescentfunction}{\nu}
\newcommand{\newtondescent}[2]{\newtondescentfunction({#1};{#2})}
\newcommand{\newtondescentblank}[1]{\newtondescent{#1}{.}}
%\newcommand{\Projection}[2]{P_{#1} \[{#2} \] }
\newcommand{\yy}{y}
\newcommand{\yyprime}{\yy^\prime}
\newcommand{\yysol}{\yy^\star}
\newcommand{\yysoli}[1]{\yysol_{#1}}
\newcommand{\yyi}[1]{\yy_{#1}}
\newcommand{\yykj}[2]{\yyk{#1}({#2})}
\newcommand{\yykji}[3]{\yyk{#1}_{#3}({#2})}
\newcommand{\zzi}[1]{\zz_{#1}}
\newcommand{\zzsol}{\zz^\star}
\newcommand{\zzsoli}[1]{\zzsol_{#1}}
\newcommand{\barxx}{\bar \xx}
\newcommand{\baryy}{\bar \yy}
\newcommand{\barzz}{\bar \zz}
\newcommand{\xxKKT}{\xx}
\newcommand{\xxKKTi}[1]{\xxKKT_{#1}}
\newcommand{\yyKKT}{\yy}
\newcommand{\yyKKTi}[1]{\yyKKT_{#1}}
\newcommand{\zzKKT}{\zz}
\newcommand{\zzKKTi}[1]{\zzKKT_{#1}}

%\newcommand{\buffj}[1]{\buff({#1})}
%\newcommand{\buffji}[2]{\buff_{#2}({#1})}
\newcommand{\buffj}[1]{\buff^{#1}}
\newcommand{\buffji}[2]{\buff_{#2}^{#1}}
\newcommand{\yyj}[1]{y^{#1}}
\newcommand{\yyjxa}[3]{\yyj{#1} ({#2},{#3})}
\newcommand{\yyjxai}[4]{\yyj{#1}_{#4} ({#2},{#3})}
\newcommand{\dx}{h}
\newcommand{\dxj}[1]{\dx_{#1}}

\newcommand{\Pamin}{\text{\b{$\Pa$}}} %{\bar \Pa}

\newcommand{\conditionnumber}[1]{\kappa({#1})}

%\newcommand{\Nxi}[2]{N^{#1}_{#2}}
%\newcommand{\Ei}[1]{\tilde N_{#1}}
%\newcommand{\tilde}[1]{\tilde N_{#1}}
\newcommand{\transmitxij}[3]{\text{Transmit }{#1}\text{ to all }{#3} \in  \Ni{{#2}} }
\newcommand{\transmitxbacki}[2]{\text{Transmit }{#1}\text{ to  }{#2}}
\newcommand{\algotransmitxij}[3]{\text{\bf{transmit} }{#1}\text{ \bf{to all} }{#3} \in  \Ni{{#2}} }
\newcommand{\algotransmitxbacki}[2]{\text{\bf{transmit} }{#1}\text{ \bf{to}  }{#2}}
%\newcommand{\execute}[2]{\text{Execute in all }{#2} \in  \Nitilde{{#1}} }
%\newcommand{\executeandi}[3]{\text{Execute in all }{#3} \in  \{ {#1} \} \cup\Nitilde{{#2}} }
\newcommand{\Niandi}[2]{\Ni{{#2}} \cup  \{ {#1} \} }
\newcommand{\interset}[2]{\tilde \setofneighbours_{{#1}{#2}}}
\newcommand{\neighbourloop}[2]{{#2} \in  \Ni{{#1}} }
\newcommand{\execute}[2]{\text{Execute in all }{#2} \in  \Ni{{#1}} }
\newcommand{\executeandi}[3]{\text{Execute in all }{#3} \in  \Niandi{#1}{#2} }
\newcommand{\primaldescenti}[2]{primal\_descent({#1};{#2})}
%\newcommand{\dualarmijoi}[5]{dual\_armijo\_step({#1},{#3},{#4},{#5};{#2})}
\newcommand{\dualarmijoi}[5]{partial\_projected\_gradient\_descent({#1},{#3},{#4},{#5};{#2})}
\newcommand{\dualarmijoishort}[5]{partial\_proj\_gradient\_descent({#1},{#3},{#4},{#5};{#2})}
\newcommand{\stochdualarmijoki}[6]{stochastic\_dual\_armijo\_step({#1},{#2},{#4},{#5},{#6};{#3})}
\newcommand{\dualnewtoni}[4]{dual\_newton\_step({#1},{#3},{#4};{#2})}
\newcommand{\objectivei}[2]{\objectivefunction_{#2}({#1})}
\newcommand{\objectivefunctioni}[1]{\objectivefunction_{#1}}

\newcommand{\LVij}[2]{\Rconst_{{#1}{#2}}}
\newcommand{\Lvi}[1]{\cconst_{#1}}
\newcommand{\xxsoli}[2]{\xxi{#1}^*({#2})}

\newcommand{\deltadual}{\Delta}%^{\dualfunction}}
\newcommand{\dualzero}{\Sigma}%^{\dualfunction}}
\newcommand{\deltaduali}[1]{\delta_{#1}}
\newcommand{\hatlamb}{\hat \llamb}
\newcommand{\hatlambi}[1]{\hatlamb_{#1}}
\newcommand{\while}[1]{\text{Repeat while }{#1}}
\newcommand{\ifloop}[1]{{If }{#1}}
\newcommand{\elseloop}[1]{{Else }{#1}}


%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%

\newcommand{\smallpm}{\!\pm\!}
\newcommand{\smallx}{\!\times\!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\notxafunction}{\bar{\notx}}
\newcommand{\notxa}[1]{\notxafunction({#1})}
\newcommand{\notxkafunction}[1]{\notxafunction^{#1}}
\newcommand{\notxka}[2]{\notxkafunction{#1}({#2})}
\newcommand{\notxi}[1]{\notx_{#1}}
\newcommand{\notxk}[1]{\notx^{#1}}
\newcommand{\notxki}[2]{\notx^{#1}_{#2}}
\newcommand{\notxij}[2]{(\notxi{#1})_{#2}}
\newcommand{\notyi}[1]{\noty_{#1}}

%%%%%%%%%%%%%%%%%%%%

\newcommand{\cccahide}[2]{#1}
\newcommand{\shorten}[2]{#1}
\newcommand{\acchide}[2]{#2}
\newcommand{\accshorthide}[2]{#1}

\newcommand{\interior}[1]{\text{int}({#1})}

\newcommand{\trsp}{\prime}

\newcommand{\sepa}{\hspace{-2.5mm} & \hspace{-2.5mm} }
\newcommand{\SGsymbol}{\text{SG}}
\newcommand{\DAsymbol}{\text{DA}}
\newcommand{\AIsymbol}{\text{AI}}
\newcommand{\ANsymbol}{\text{AN}}

\newcommand{\tableaufunction}{\tau}
\newcommand{\tableau}[1]{\tableaufunction ({#1})}
\newcommand{\tableausymbol}[2]{\tableaufunction^{#1}({#2})}
\newcommand{\tableaugapfunction}{\varphi}
\newcommand{\tableaugap}[1]{\tableaugapfunction ({#1})}
\newcommand{\tableaugapsymbol}[2]{\tableaugapfunction^{#1}({#2})}
\newcommand{\tableausamplefunction}{\vartheta}
\newcommand{\tableausample}[1]{\tableausamplefunction ({#1})}
\newcommand{\tableausamplesymbol}[2]{\tableausamplefunction^{#1}({#2})}
\newcommand{\tabmean}[1]{\bar {\tableaufunction}({#1})}
%\newcommand{\tabmean}[1]{\mu_{\tableaufunction}({#1})}
\newcommand{\tabstd}[1]{\sigma_{\tableaufunction}({#1})}
\newcommand{\tabmeansymbol}[2]{\mu_{\tableaufunction}^{#1}({#2})}
\newcommand{\tabstdsymbol}[2]{\sigma_{\tableaufunction}^{#1}({#2})}
\newcommand{\messagepassingfunction}{\phi}
\newcommand{\messagepassing}[1]{\messagepassingfunction ({#1})}
%\newcommand{\mpmean}[1]{\mu_{\messagepassingfunction}({#1})}
\newcommand{\mpmean}[1]{\bar {\messagepassingfunction}({#1})}
\newcommand{\mpstd}[1]{\sigma_{\messagepassingfunction}({#1})}


\newcommand{\thinampersand}{\hspace{-1.5mm} & \hspace{-1.5mm}}

\newcommand{\arginf}{{\arg}\,\inf}
\newcommand{\argsup}{{\arg}\,\sup}
\newcommand{\underarginf}[1]{\underset{{#1}}{\arginf}\, }
\newcommand{\underargsup}[1]{\underset{{#1}}{\argsup}\, }

\newcommand{\Gobjective}{f^0}
\newcommand{\Lobjectivei}[1]{\Gobjective_{#1}}
\newcommand{\horizontaline}[1]{\vspace{-0mm} \centerline{\begin{tabular}{c}\ \hspace{80mm} \ \\ \hline \end{tabular}}\vspace{-0mm}}

\newcommand{\qq}{q}
\newcommand{\rr}{r}
%\newcommand{\Gx}{{\mathbf{x}}}
%\newcommand{\Gy}{{\mathbf{y}}}
%\newcommand{\GX}{{\mathbf{X}}}
\newcommand{\Gx}{{x}}
\newcommand{\Gy}{{y}}
\newcommand{\GX}{{X}}
\newcommand{\Lxi}[1]{\Gx_{#1}}
\newcommand{\LXi}[1]{\GX_{#1}}
\newcommand{\Lyi}[1]{\Gy_{#1}}
%\newcommand{\qq}{x}
%\newcommand{\rr}{\bar x}
%\newcommand{\yy}{\bar {\bar x }}
\newcommand{\zz}{\hat {\bar x }}

\newcommand{\rij}[2]{\rr_{#1 #2}}%{r_{#1 #2}}
\newcommand{\yij}[2]{\yy_{#1 #2}} %y
\newcommand{\zijk}[3]{{\zz^{#1}_{#2 #3}}} %z
\newcommand{\qi}[1]{\qq_{#1}}
\newcommand{\yijk}[3]{{\yy^{#1}_{#2 #3}}} %z


\newcommand{\upsiloni}[1]{\upsilon_{#1}}
\newcommand{\gammaij}[2]{\gamma_{#1 #2}}
\newcommand{\etaijk}[3]{{\eta^{#1}_{#2 #3}}}

\newcommand{\ffi}[1]{f_{#1}}
\newcommand{\hij}[2]{h_{#1 #2}}
\newcommand{\gijk}[3]{{g^{#1}_{#2 #3}}}

\newcommand{\Ni}[1]{\setofneighbours_{#1}}
\newcommand{\Nxi}[2]{N^{#1}_{#2}}
\newcommand{\Nitilde}[1]{\tilde N_{#1}}
\newcommand{\Exi}[2]{\mathcal{N}^{#1}_{#2}}
\newcommand{\Ei}[1]{\mathcal{N}_{#1}}
\newcommand{\KKK}{\bar k}

%\renewcommand{\Pi}[1]{\mathcal{P}_{#1}}
\newcommand{\Dij}[2]{\mathcal{D}_{#1 #2}}
\newcommand{\Sij}[2]{\mathcal{S}_{#1 #2}}

\newcommand{\Eij}[2]{e_{#1 #2}} %E
\newcommand{\Eijk}[3]{{e_{#2 #3}}} %E
%\newcommand{\Eijk}[3]{{e^{#1}_{#2 #3}}} %E
\newcommand{\Eijkl}[4]{{e^{#1}_{#2 #3 #4}}} %E
\newcommand{\Rij}[2]{\rr^{{max}}_{#1 #2}} %E
\renewcommand{\Si}[1]{s_{#1}} % conflict with package {algorithm2e}
%\newcommand{\Si}[1]{s_{#1}}
\newcommand{\generation}{s}
\newcommand{\Bi}[1]{b_{#1}}
\newcommand{\resource}{b}
%\newcommand{\QQ}{\mathbf{a}}
%\newcommand{\QQ}{{a}}
\newcommand{\QQ}{{z}}

\newcommand{\SNR}{S\!N\!R}
\newcommand{\FB}{F\!B}
%\newcommand{\FB}{C\!S\!I}
\newcommand{\vvvfill}{\vspace{20cm} \ }
%\newrgbcolor{efface}{0.6 0.6 0.6}
%\newcommand{\trigri}{\textcolor{efface}{$\blacktriangleright$}}
%\newcommand{\tribla}{\textcolor{black}{$\blacktriangleright$}}

\newcommand{\Tee}{\mathcal{T}}
\newcommand{\Pee}{\mathcal{P}}
\newcommand{\Kee}{\mathcal{K}}
\newcommand{\Mee}{\mathcal{M}}
\newcommand{\Dee}{\Mee}
\newcommand{\Nee}{\mathcal{N}}
\newcommand{\See}{\mathcal{S}}

\newcommand{\Power}[1]{P_{#1}}
\newcommand{\Gain}[1]{G_{#1}}
\newcommand{\Area}[1]{A_{#1}}
\newcommand{\Height}[1]{l_{#1}}
\newcommand{\Noise}[1]{N_{#1}}

\newcommand{\pout}{p_{out}}
\newcommand{\pfail}{P_{fail}}
\newcommand{\Ebf}{E_{bf}}
\newcommand{\ho}[1]{h_{ \lbrack #1 \rbrack } }
\newcommand{\go}[1]{g_{ \lbrack #1 \rbrack } }
\newcommand{\xo}[1]{x_{ \lbrack #1 \rbrack } }

\newcommand{\Tnet}{t_{net}}
\newcommand{\Tneti}[1]{\Tnet({#1})}
\newcommand{\Ti}[1]{t_{#1}}
\newcommand{\Poweri}[1]{p_{#1}}
\newcommand{\Sbc}{S}%^{bc}}
\newcommand{\Sbf}{S}%^{bf}}


\newcommand{\BAR}{\hspace{-2mm} & \hspace{-2mm}}%^{bf}}
\newcommand{\BARR}{\hspace{-1.5mm} & \hspace{-1.5mm}}%^{bf}}
\newcommand{\temporary}[1]{\textcolor{green}{\emph{#1}}}

\newcommand{\ypp}{y_p}
%\newcommand{\xx}{\mathbf{x}}

\newcommand{\zero}[1]{o({#1})}

\newcommand{\eps}{e}
\newcommand{\EPS}{$\epsilon$-subgradient}
\newcommand{\prox}{p}
\newcommand{\PROX}{primal proximal}
\newcommand{\pmom}{pm}
\newcommand{\PMOM}{PMOM}
\newcommand{\pcpm}{pc}
\newcommand{\PCPM}{PCPM}

\newcommand{\feps}{f^\eps}
\newcommand{\fprox}{f^\prox}
\newcommand{\lprox}{l^\prox}
\newcommand{\laugmented}{F^\prox}
\newcommand{\lproxprox}{L^\prox}

\newcommand{\lpar}{\phi}
\newcommand{\lparam}[2]{\lpar^{#1}_{#2}}
\newcommand{\lpcpm}[1]{\lparam{\pcpm}{#1}}
\newcommand{\subglambdagen}{\sigma}
\newcommand{\subgmugen}{\tau}
\newcommand{\subglambda}[1]{\subglambdagen^{#1}}
\newcommand{\subgmu}[1]{\subgmugen^{#1}}
%\newcommand{\lpr}[1]{{\phi\prime_{#1}}}
\newcommand{\transmit}[1]{\text{Transmit }{#1}\text{ to all }j \in  \Ni{i} } %\subset \Nxi{\KKK}{i}} %}{k}\text{-neighbours}}
\newcommand{\primalrecovery}{{{primal\_variables}}}
\newcommand{\primalrecoveryfunction}[2]{\primalrecovery({#1},{#2})}
\newcommand{\dualsubgradientdescent}{{{dual\_sg}}} %
\newcommand{\dualsubgradientdescentfunction}[7]{\dualsubgradientdescent({#1},{#2},({#3},{#4}),{#5},{#6},{#7})}
\newcommand{\epsilonsubgradient}{{{epsilon\_sg}}}
\newcommand{\epsilonsubgradientfunction}[5]{\epsilonsubgradient({#1},{#2},{#3},{#4},{#5})}
\newcommand{\primalproximal}{{{primal\_proximal}}}
\newcommand{\primalproximalfunction}[5]{\primalproximal({#1},{#2},{#3},{#4},{#5})}%,{#5})}
\newcommand{\proximalmethodofmultipliers}{{{pmom}}}
\newcommand{\proximalmethodofmultipliersfunction}[4]{\proximalmethodofmultipliers({#1},{#2},{#3},{#4})}%,{#5})}
\newcommand{\predictorcorrectorproximalmultiplier}{{{pcpm}}}
\newcommand{\predictorcorrectorproximalmultiplierfunction}[2]{\predictorcorrectorproximalmultiplier({#1},{#2})}%,{#3})}%,{#4})}



%%%%%%


\newcommand{\MMprime}{\tilde\MM}

\newcommand{\firstindex}{\hat i}
\newcommand{\firstindexk}[1]{\firstindex^{#1}}
\newcommand{\firstdescent}{\gamma}
\newcommand{\firstdescenti}[1]{\firstdescent_{#1}}
\newcommand{\firstdescentk}[1]{\firstdescent^{#1}}
\newcommand{\firstdescentki}[2]{\firstdescent^{#1}_{#2}}

\newcommand{\setofPas}{A}
\newcommand{\Pmmax}{\bar{\Pm}}
\newcommand{\searchfactor}{\alpha}
\newcommand{\boundary}[1]{\delta {#1}}
\newcommand{\manifoldfunction}{\bar \setoflambdas}
\newcommand{\manifoldifunction}[1]{\manifoldfunction_{#1}}
\newcommand{\manifold}[1]{\manifoldfunction({#1})}
\newcommand{\manifoldi}[2]{\manifoldifunction{#1}({#2})}
\newcommand{\epsonefour}{\epsilon}
\newcommand{\epsonefourPa}[1]{\epsonefour ({#1})}
%\newcommand{\epsone}{\epsilon^\prime}
%\newcommand{\epsone}{\epsonefour}
\newcommand{\epsfour}{\epsilon^\delta}
\newcommand{\epsout}{\zeta}
\newcommand{\epsoutPa}[1]{\epsout ({#1})}
\newcommand{\epsepsonefour}{\bar \zeta}
\newcommand{\epsepsonefourPa}[1]{\epsepsonefour ({#1})}
\newcommand{\epsstar}{\epsilon^\star}
\newcommand{\epsstarPa}[1]{\epsstar ({#1})}
\newcommand{\epsfinal}{\epsilon}
\newcommand{\ball}[2]{B({#1},{#2})}
\newcommand{\closedball}[2]{\bar B({#1},{#2})}
\newcommand{\manifoldball}[2]{\bar B({#1},{#2})}
\newcommand{\ellipsoidfunction}{z}
\newcommand{\ellipsoid}[1]{\ellipsoidfunction({#1})}
\newcommand{\ellipsoidPafunction}[1]{\ellipsoidfunction^{#1}}
\newcommand{\ellipsoidPa}[2]{\ellipsoidfunction^{#1}({#2})}
%\newcommand{\ellipsoidPa}[2]{\ellipsoidfunction({#1};{#2})}
\newcommand{\genericepsilon}{\omega}
\newcommand{\llambellipsoid}{\xi}

\newcommand{\makematrix}[4]{\left(\begin{array}{cc} {#1} & {#2} \\ {#3} & {#4} \end{array}\right)}
\newcommand{\makevector}[2]{\left(\begin{array}{c} {#1} \\ {#2} \end{array}\right)}

\newcommand{\pseudoH}{\tilde H}
\newcommand{\pseudoQ}{\tilde Q}
\newcommand{\pseudoI}{I}
\newcommand{\pseudok}{\kappa}
\newcommand{\pseudoamin}{\Pa^{min}}
\newcommand{\pseudoalpha}{\alpha}


\newcommand{\DSpsifunction}{\psi}
\newcommand{\DSpsiifunction}[1]{\DSpsifunction_{#1}}
\newcommand{\DSpsii}[2]{\DSpsiifunction{#1}({#2})}
\newcommand{\DScoeffunction}{\alpha}
\newcommand{\DScoefifunction}[1]{\DScoeffunction_{#1}}
\newcommand{\DScoefi}[2]{\DScoefifunction{#1} ({#2})}

\newcommand{\DSsafety}{\epsilon}

\newcommand{\reg}{q}
\newcommand{\regbis}{r}
\newcommand{\nreg}{\reg^\star}
%\newcommand{\NDr}{r^\star}
\newcommand{\NDr}{\HYBrhomax}
\newcommand{\NDu}{u}
\newcommand{\NDalpha}{\alpha}
\newcommand{\NDjkit}[3]{j({#3})}
\newcommand{\NDtki}[2]{t}
\newcommand{\NDtau}{\tau}
\newcommand{\NDrho}{\rho}


\newcommand{\NDhessianfunction}{h} %{\overrightarrow H}
\newcommand{\NDhessiank}[1]{\NDhessianfunction^{#1}}
\newcommand{\NDhessiankx}[2]{\NDhessiank{#1}({#2})}
\newcommand{\NDhessiankxi}[3]{\NDhessiank{#1}_{#3}({#2})}
\newcommand{\NDhessianki}[2]{\NDhessiank{#1}_{#2}}
\newcommand{\NDhessiantildefunction}{\tilde \NDhessianfunction} %{\overrightarrow H}
\newcommand{\NDhessiantildek}[1]{\NDhessiantildefunction^{#1}}
\newcommand{\NDhessiantildekx}[2]{\NDhessiantildek{#1}({#2})}
\newcommand{\NDhessiantildekxi}[3]{\NDhessiantildek{#1}_{#3}({#2})}
\newcommand{\NDhessiantildeki}[2]{\NDhessiantildek{#1}_{#2}}
\newcommand{\NDalphakit}[3]{\NDalpha({#3})}
\newcommand{\NDrhok}[1]{\NDrho({#1})}
\newcommand{\NDindexk}[1]{\NDrho({#1})}
\newcommand{\NDhood}{\hood}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\dimx}{\NN}
\newcommand{\Rconst}{C}
\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\REALone}{\mathbb{R}}
\newcommand{\REAL}[1]{\REALone^{#1}}
\newcommand{\REALonepinfty}{(-\infty,\infty]} %{\REALone\cup\{\infty\}}
\newcommand{\REALoneminfty}{[-\infty,\infty)} %{\REALone\cup\{-\infty\}}
\newcommand{\REALonepminfty}{[-\infty,\infty]} %{\REALone\cup\{-\infty,\infty\}}
\newcommand{\LIP}[1]{\textnormal{Lip}({#1})}
\newcommand{\CON}[1]{\textnormal{Con}({#1})}
\newcommand{\CDone}[1]{\mathbb{C}({#1})}
\newcommand{\CD}[2]{\mathbb{C}^{#1}({#2})}
\newcommand{\CCL}[1]{\CCLone({#1})}
\newcommand{\minimisefunction}{\text{\textup{minimise}}}
\newcommand{\maximisefunction}{\text{\textup{maximise}}}
\newcommand{\minimise}[1]{\underset{#1}{\minimisefunction{} \ }}
\newcommand{\maximise}[1]{\underset{#1}{\maximisefunction{} \ }}
\newcommand{\minimisenolimits}[1]{{\minimisefunction}_{#1}}
\newcommand{\maximisenolimits}[1]{{\maximisefunction}_{#1}}
\newcommand{\st}{\text{\textup{s. t.}}}
\newcommand{\subjectto}{\text{\textup{subject to }}}
\newcommand{\objectivefunction}{f}
\newcommand{\objective}[1]{\objectivefunction(#1)}
\newcommand{\oG}{D} % Q
\newcommand{\oGi}[1]{\oG_{#1}} % Q
\newcommand{\og}{b}
\newcommand{\ogi}[1]{\og_{#1}}
\newcommand{\lagrangianfunction}{l}
\newcommand{\lagrangian}[2]{\lagrangianfunction({#1},{#2})}
\newcommand{\lagrangianifunction}[1]{\lagrangianfunction_{#1}}
\newcommand{\lagrangiani}[3]{\lagrangianifunction{#1}({#2},{#3})}
\newcommand{\lagrangianlambdafunction}{\tilde l}
\newcommand{\lagrangianilambdafunction}[1]{\lagrangianlambdafunction_{#1}}
\newcommand{\lagrangianlambda}[4]{\lagrangianlambdafunction ({#1},{#2};{#3},{#4})}
\newcommand{\lagrangianilambda}[5]{\lagrangianilambdafunction{#1} ({#2},{#3};{#4},{#5})}
\newcommand{\dualfunction}{g}
\newcommand{\dual}[1]{\dualfunction(#1)}
\newcommand{\duali}[2]{\dualfunction_{#1}({#2})}
\newcommand{\dualifunction}[1]{\dualfunction_{#1}}
\newcommand{\unconstraineddualfunction}{\hat \dualfunction}
\newcommand{\unconstraineddualifunction}[1]{\unconstraineddualfunction_{#1}}
\newcommand{\unconstraineddual}[2]{\unconstraineddualfunction({#1};{#2})}
\newcommand{\unconstrainedduali}[3]{\unconstraineddualifunction{#1}({#2};{#3})}
\newcommand{\lambdasolfunction}{\bar \llamb^*}
\newcommand{\lambdasol}[1]{\lambdasolfunction(#1)}
\newcommand{\lambdaifunction}[1]{\lambdafunction_{#1}}
\newcommand{\xsolbarfunction}{\bar x^*}
\newcommand{\xsolbar}[1]{\xsolbarfunction({#1})}
\newcommand{\xlambdai}[2]{\lambdaifunction{#1}(#2)}
\newcommand{\Xsolfunction}{X^*}
\newcommand{\xsolfunction}{x^*}
\newcommand{\xsol}[1]{\xsolfunction(#1)}
\newcommand{\xsolifunction}[1]{\xsolfunction_{#1}}
\newcommand{\xsoli}[2]{\xsolifunction{#1}(#2)}
\newcommand{\lamb}{\bar \llamb}
\newcommand{\lambPa}[1]{\lamb ({#1})}
\newcommand{\lambi}[1]{\lamb_{#1}}
\newcommand{\lambPai}[2]{\lamb_{#2}({#1})}
\newcommand{\nbedges}{s}
\newcommand{\Edges}{S}
\newcommand{\neighbourhood}[2]{\mathcal{N}^{#1}_{#2}}
\newcommand{\xlamb}{\bar x}
\newcommand{\xlambi}[1]{\xlamb_{#1}}
\newcommand{\xsolzero}[1]{\xi^0(#1)}
\newcommand{\xsollambdafunction}{\xi}
\newcommand{\xsolilambdafunction}[1]{\xsollambdafunction_{#1}}
\newcommand{\xsollambda}[2]{\xsollambdafunction({#1};{#2})}
\newcommand{\xsolilambda}[3]{\xsolilambdafunction{#1}({#2};{#3})}
%\newcommand{\xsollamblambdafunction}[2]{\hat \xi_{{#1},{#2}}}
%\newcommand{\xsollamblambda}[3]{\xsollamblambdafunction{#1}{#2}(#3)}
\newcommand{\xsollamblambdafunction}{\hat \xi}
\newcommand{\xsolilamblambdafunction}[1]{\xsollamblambdafunction_{#1}}
\newcommand{\xsollamblambda}[3]{\xsollamblambdafunction ({#1},{#2};{#3})}
\newcommand{\xsolilamblambda}[4]{\xsolilamblambdafunction{#1} ({#2},{#3};{#4})}
\newcommand{\gammai}[1]{\gamma_{#1}}
\newcommand{\gammasollambdafunction}{\gamma^*}
\newcommand{\gammasolilambdafunction}[1]{\gammasollambdafunction_{#1}}
\newcommand{\gammasollambda}[2]{\gammasollambdafunction({#1};{#2})}
\newcommand{\gammasolilambda}[3]{\gammasolilambdafunction{#1}({#2};{#3})}
%\newcommand{\lambdasetk}[1]{\lambdaset^{#1}}
\newcommand{\lambdasetk}[1]{\tilde \lambdaset}
\newcommand{\intlambdasetk}[1]{\lambdaset_0^{#1}}
\newcommand{\lambdasetzero}{\lambdasetk{0}}
\newcommand{\lambdasetlambda}[1]{\lambdasetk{\delta}({#1})}
\newcommand{\intlambdasetlambda}[1]{\intlambdasetk{\delta}({#1})}
%\newcommand{\Xsetlambda}[1]{X^{\delta}({#1})}
\newcommand{\Xsetlambda}[1]{\tilde X({#1})}
\newcommand{\Xsetilambda}[2]{\tilde X_{#1}({#2})}
\newcommand{\bordersetlambda}[1]{B({#1})}

\newcommand{\jacobian}[2]{\jacobianfunction{#1}({#2})}
\newcommand{\jacobiani}[3]{\jacobianifunction{#1}{#2}({#3})}
\newcommand{\jacobianij}[4]{\jacobianifunction{#1}{#2}{#3}({#4})}

\newcommand{\jacobiantildefunction}[1]{J^{#1}}
\newcommand{\jacobiantilde}[2]{\jacobianfunction{#1}({#2})}
\newcommand{\jacobiantildeifunction}[2]{\jacobianfunction{#1}_{#2}}
\newcommand{\jacobiantildei}[3]{\jacobianifunction{#1}{#2}({#3})}
\newcommand{\jacobiantildeijfunction}[3]{\jacobianfunction{#1}_{#2}{#3}}
\newcommand{\jacobiantildeij}[4]{\jacobianifunction{#1}{#2}{#3}({#4})}
\newcommand{\hessian}[2]{\hessianfunction{#1}(#2)}
\newcommand{\hessiani}[3]{\hessianifunction{#1}{#2}(#3)}
\newcommand{\hessianij}[4]{\left(\hessianifunction{#1}{#2}(#4)\right)_{{#3}}}
\newcommand{\hessiantilde}[2]{\hessiantildefunction{#1}(#2)}
\newcommand{\hessiantildei}[3]{\hessiantildeifunction{#1}{#2}(#3)}
\newcommand{\hessiantildeij}[4]{\left(\hessiantildeifunction{#1}{#2}(#4)\right)_{{#3}}}
\newcommand{\deltataylor}{\delta}
\newcommand{\deltataylortilde}{\tilde \delta}
%\newcommand{\hessiantilde}[1]{\tilde H_{#1}}
\newcommand{\gradienttilde}[1]{\tilde \grad_{\!{#1}}}
\newcommand{\gradtilde}{\tilde \grad}
\newcommand{\gradftilde}{\tilde \grad \dualfunction}
\newcommand{\gradfxtilde}[1]{\gradftilde ( {#1} )}
\newcommand{\graditilde}[1]{\tilde \grad_{\! #1}}
\newcommand{\gradfitilde}[1]{\graditilde{#1}\dualfunction}
\newcommand{\gradfxitilde}[2]{\gradfitilde{#2} ( {#1} )}
\newcommand{\LCsetoflambdas}{\tilde \setoflambdas}
\newcommand{\LCsetoflambdask}[1]{\LCsetoflambdas^{#1}}
\newcommand{\LCsetoflambdasi}[1]{\LCsetoflambdas_{#1}}
\newcommand{\LCsetoflambdaski}[2]{\LCsetoflambdask{#1}_{#2}}
\newcommand{\ksc}{\bar k}
\newcommand{\kscbis}{\hat k}
\newcommand{\kscter}{\tilde{k}}
\newcommand{\tsc}{\bar t}
\newcommand{\LCScale}{\tilde T} %obsolete
\newcommand{\LCScalei}[1]{\LCScale_{#1}}
\newcommand{\LCScalek}[1]{\LCScale^{#1}}
\newcommand{\LCScaleki}[2]{{\LCScalek{#1}_{#2}}}
\newcommand{\LCScaleix}[2]{\LCScalei{#1}({#2})}
\newcommand{\LCScalex}[1]{\LCScale({#1})}
\newcommand{\LCScaleq}[1]{\LCScale^{(#1)}}
\newcommand{\Scaleq}[1]{\Scale^{(#1)}}
\newcommand{\LCScaleqx}[2]{\LCScaleq{#1}({#2})}
\newcommand{\Scaleqx}[2]{\Scaleq{#1}({#2})}
\newcommand{\LCsScale}{\tilde T}
\newcommand{\LCsScalei}[1]{\LCsScale_{#1}}
\newcommand{\LCsScaleix}[2]{\LCsScalei{#1}({#2})}
\newcommand{\LCsScalex}[1]{\LCsScale({#1})}
\newcommand{\LCsScaleij}[2]{\LCsScale_{{#1}{#2}}}
\newcommand{\LCsScaleijx}[3]{\LCsScaleij{#1}{#2}({#3})}



\newcommand{\HYBd}{d}
\newcommand{\HYBm}{m}
\newcommand{\HYBgammai}[1]{\gamma^\star_{#1}}
\newcommand{\HYBgammaid}[2]{\HYBgammai{#1}({#2})}
\newcommand{\HYBGammai}[1]{\Gamma^\star_{#1}}
\newcommand{\HYBrhomax}{\bar \HYBrho}
\newcommand{\HYBrhok}[1]{\HYBrho({#1})}


\newcommand{\NDScaler}[1]{T^{#1}}
\newcommand{\NDScaleri}[2]{\NDScaler{#1}_{#2}}
\newcommand{\NDScalerix}[3]{\NDScaleri{#1}{#2}({#3})}
\newcommand{\NDScalerx}[2]{\NDScaler{#1}({#2})}
\newcommand{\NDsScaler}[1]{S^{#1}}
\newcommand{\NDsScaleri}[2]{\NDsScaler{#1}_{#2}}
\newcommand{\NDsScalerix}[3]{\NDsScaleri{#1}{#2}({#3})}
\newcommand{\NDsScalerx}[2]{\NDsScaler{#1}({#2})}
\newcommand{\NDtildeScaler}[1]{\tilde \Scale^{#1}}
\newcommand{\NDtildeScaleri}[2]{\NDtildeScaler{#1}_{#2}}
\newcommand{\NDtildeScalerix}[3]{\NDtildeScaleri{#1}{#2}({#3})}
\newcommand{\NDtildeScalerx}[2]{\NDtildeScaler{#1}({#2})}
\newcommand{\NDtildesScaler}[1]{\tilde S^{#1}}
\newcommand{\NDtildesScaleri}[2]{\NDtildesScaler{#1}_{#2}}
\newcommand{\NDtildesScalerix}[3]{\NDtildesScaleri{#1}{#2}({#3})}
\newcommand{\NDtildesScalerx}[2]{\NDtildesScaler{#1}({#2})}


\newcommand{\LChood}{\tilde \hood}
\newcommand{\LChoodi}[1]{\LChood_{#1}}
\newcommand{\LClamb}{\tilde \llamb}
\newcommand{\LClambi}[1]{\LClamb_{#1}}
\newcommand{\LClambk}[1]{\LClamb^{#1}}
\newcommand{\LClambki}[2]{\LClamb^{#1}_{#2}}
\newcommand{\LClambconv}{\tilde \llamb^\star}
\newcommand{\LClambconvi}[1]{\LClambconv_{#1}}
\newcommand{\LCmui}[1]{\LCmu_{#1}}
\newcommand{\LClambcs}{\tilde \llamb^*}
\newcommand{\LClambcsi}[1]{\LClambcs_{#1}}
\newcommand{\LCdfunction}{\tilde d}
\newcommand{\LCd}[1]{\LCdfunction ({#1})}
\newcommand{\LCdifunction}[1]{\LCdfunction_{#1}}
\newcommand{\LCdi}[2]{\LCdifunction{#1} ({#2})}
\newcommand{\mmudy}[2]{\mmu ({#1},{#2})}
\newcommand{\LCHfunction}{\tilde Z}
\newcommand{\LCH}[2]{\LCHfunction ({#1},{#2})}
\newcommand{\LCHifunction}[1]{\LCHfunction_{#1}}
\newcommand{\LCHi}[3]{\LCHifunction{#1}({#2},{#3})}
\newcommand{\LCHbisfunction}{\tilde z}
\newcommand{\LCHbis}[1]{\LCHbisfunction({#1})}
\newcommand{\globalDfunction}{D}
\newcommand{\globalD}[1]{\globalDfunction({#1})}
\newcommand{\globalDij}[3]{\globalDfunction_{{#2}{#3}}({#1})}
\newcommand{\globalLfunction}{L}
\newcommand{\globalL}[1]{\globalLfunction ({#1})}
\newcommand{\globalLij}[3]{\globalLfunction_{{#2}{#3}}({#1})}
\newcommand{\LCDfunction}{\tilde \globalDfunction}
\newcommand{\LCD}[1]{\LCDfunction ({#1})}
\newcommand{\LCDij}[3]{\LCDfunction_{{#2}{#3}}({#1})}
\newcommand{\LCLfunction}{\tilde \globalLfunction}
\newcommand{\LCL}[1]{\LCLfunction ({#1})}
\newcommand{\LCLij}[3]{\LCLfunction_{{#2}{#3}}({#1})}
\newcommand{\LCAfunction}{\tilde A}
\newcommand{\LCA}[1]{\LCAfunction ({#1})}
\newcommand{\globalMfunction}{R}
\newcommand{\LCMfunction}{\tilde{\globalMfunction}}
\newcommand{\LCMSfunction}{\LCMfunction^{S}}
%\newcommand{\LCM}[1]{\LCMfunction ({#1})}
\newcommand{\LCM}[1]{\LCMSfunction ({#1})}
\newcommand{\LCMJfunction}{\LCMfunction^{\mapping}}
\newcommand{\LCMJ}[1]{\LCMJfunction ({#1})}
%\newcommand{\LCMset}[1]{\mathcal{R} ({#1})}
\newcommand{\Zmappingq}[1]{\Zmapping^{({#1})}}
\newcommand{\LCMqfunction}[1]{\LCMfunction^{\Zmappingq{#1}}}
\newcommand{\LCMq}[2]{\LCMqfunction{#1}({#2})}
\newcommand{\globalMqfunction}[1]{\globalMfunction^{\Zmappingq{#1}}}
\newcommand{\globalMq}[2]{\globalMqfunction{#1}({#2})}
\newcommand{\LCMset}[1]{\mathcal{R}^{\Smapping} ({#1})}
\newcommand{\LCMk}[2]{\LCMfunction^{\Smapping}({#1},{#2})}
%\newcommand{\LCMk}[2]{\LCMfunction^{({#1})} ({#2})}
\newcommand{\LCbarT}{\hat T}
\newcommand{\LCbarTij}[2]{\LCbarT_{{#1}{#2}}}
\newcommand{\LCbarM}{\hat M}
\newcommand{\LCbarMij}[2]{\LCbarM_{{#1}{#2}}}
\newcommand{\LChatlamb}{\hat \llamb}
\newcommand{\LCostrowA}[1]{\bar A}
\newcommand{\LCostrowD}[1]{\bar D}
\newcommand{\LCostrowE}[1]{\bar E}
\newcommand{\LCBfunction}{\tilde B}
\newcommand{\LCB}[1]{\LCBfunction ({#1})}
\newcommand{\manifoldsetoflambdas}{\setoflambdas^{\star}}
\newcommand{\manifoldsetoflambdasi}[1]{\manifoldsetoflambdas_{#1}}
\newcommand{\bijectionf}{h}
\newcommand{\bijectionfi}[1]{\bijectionf_{#1}}
\newcommand{\bijectionfix}[2]{\bijectionfi{#1}({#2})}

%%



\newcommand{\doPROJ}[1]{\bar{#1}}
\newcommand{\nonPROJlamb}{\llamb}
\newcommand{\nonPROJmu}{\mmu}
\newcommand{\nonPROJScale}{\Scale}
\newcommand{\nonPROJPa}{\Pa}
\newcommand{\PROJx}{\doPROJ{\nonPROJx}}
\newcommand{\PROJlamb}{\doPROJ{\nonPROJlamb}}
\newcommand{\PROJmu}{\doPROJ{\nonPROJmu}}
\newcommand{\PROJScale}{\doPROJ{\Scale}}
\newcommand{\PROJs}{s}
\newcommand{\PROJPa}{\Pa}
\newcommand{\PROJordering}{B}
\newcommand{\PROJviolating}{\violatingsymbol}
\newcommand{\PROJnonviolating}{\doPROJ{\PROJviolating}}
\newcommand{\PROJviolatingx}[1]{\PROJviolating({#1})}
\newcommand{\PROJnonviolatingx}[1]{\PROJnonviolating({#1})}
\newcommand{\PROJbarT}{\tilde T}
\newcommand{\PROJbarTij}[2]{\PROJbarT_{{#1}{#2}}}
\newcommand{\PROJbarM}{\tilde M}
\newcommand{\PROJbarMij}[2]{\PROJbarM_{{#1}{#2}}}
\newcommand{\PROJhatlamb}{\hat \nonPROJmu}
\newcommand{\nonPROJnu}{\nu}
\newcommand{\nonPROJsetoflambdas}{\setoflambdas}
\newcommand{\PROJsetoflambdas}{\doPROJ{\setoflambdas}}
\newcommand{\PROJI}{I}
\newcommand{\PROJdir}{d}


\newcommand{\PROJlambcs}{\tilde \llamb^*}
\newcommand{\PROJlambcsi}[1]{\PROJlambcs_{#1}}
\newcommand{\PROJdfunction}{\tilde d}
\newcommand{\PROJd}[1]{\PROJdfunction ({#1})}
\newcommand{\PROJdifunction}[1]{\PROJdfunction_{#1}}
\newcommand{\PROJdi}[2]{\PROJdifunction{#1} ({#2})}
\newcommand{\PROJHfunction}{\tilde Z}
\newcommand{\PROJH}[2]{\PROJHfunction ({#1},{#2})}
\newcommand{\PROJHifunction}[1]{\PROJHfunction_{#1}}
\newcommand{\PROJHi}[3]{\PROJHifunction{#1}({#2},{#3})}
\newcommand{\PROJHbisfunction}{\tilde z}
\newcommand{\PROJHbis}[1]{\PROJHbisfunction({#1})}
\newcommand{\PROJDfunction}{\tilde D}
\newcommand{\PROJD}[1]{\PROJDfunction ({#1})}
\newcommand{\PROJDij}[3]{\PROJDfunction_{{#2}{#3}}({#1})}
\newcommand{\PROJLfunction}{\tilde L}
\newcommand{\PROJL}[1]{\PROJLfunction ({#1})}
\newcommand{\PROJLij}[3]{\PROJLfunction_{{#2}{#3}}({#1})}
\newcommand{\PROJAfunction}{\tilde A}
\newcommand{\PROJA}[1]{\PROJAfunction ({#1})}
\newcommand{\PROJMfunction}{\tilde R}
\newcommand{\PROJM}[1]{\PROJMfunction ({#1})}
\newcommand{\PROJMJfunction}{\tilde{R}^{J}}
\newcommand{\PROJMJ}[1]{\PROJMJfunction ({#1})}
\newcommand{\PROJMset}[1]{\mathcal{R} ({#1})}
\newcommand{\PROJMk}[2]{\PROJMfunction^{({#1})} ({#2})}
\newcommand{\PROJostrowA}[1]{\bar A}
\newcommand{\PROJostrowD}[1]{\bar D}
\newcommand{\PROJostrowE}[1]{\bar E}
\newcommand{\PROJBfunction}{\tilde B}
\newcommand{\PROJB}[1]{\PROJBfunction ({#1})}

%%




\newcommand{\qhop}{q}
\newcommand{\qhopmax}{\bar q}

\newcommand{\NDDr}[2]{\LCDfunction^{#1} ({#2})}
\newcommand{\NDLr}[2]{\LCLfunction^{#1} ({#2})}
\newcommand{\NDMr}[2]{\LCMfunction^{#1} ({#2})}
\newcommand{\NDostrowAr}[2]{\LCostrowA{#2}^{#1}}
\newcommand{\NDostrowDr}[2]{\LCostrowD{#2}^{#1}}
\newcommand{\NDostrowEr}[2]{\LCostrowE{#2}^{#1}}


\newcommand{\VPA}{A}
\newcommand{\VPbarA}{\bar A}
\newcommand{\VPD}{D}
\newcommand{\VPn}{m}
\newcommand{\VPI}{I}
\newcommand{\VPa}{v}
\newcommand{\VPai}[1]{\VPa_{#1}}
\newcommand{\VPl}{l}
\newcommand{\VPli}[1]{\VPl_{#1}}
\newcommand{\VPk}{k}
\newcommand{\VPi}{i}
\newcommand{\VPlambda}{\lambda}
\newcommand{\VPlamb}{\bar \VPlambda}



\newcommand{\ac}{a}
\newcommand{\bc}{\bar x}
\newcommand{\aci}[1]{\ac^{#1}}
\newcommand{\bci}[1]{\bc_{#1}}
\newcommand{\Acmatrix}{A}
\newcommand{\Acmatrixi}[2]{\Acmatrix_{#1}({#2})}
\newcommand{\Acorthogbase}{A^\star}
\newcommand{\Acorthog}{{\Acorthogbase}}
\newcommand{\Acorthogi}[2]{{\Acorthogbase_{#1}({#2})}}
\newcommand{\Acfull}{\tilde A}
\newcommand{\Acfulli}[2]{\Acfull_{#1}({#2})}
\newcommand{\lambdamaxzero}{\lambda_0^{max}}
\newcommand{\hpset}[1]{N({#1})}
\newcommand{\smallhpset}[1]{H({#1})}
\newcommand{\projectedmatrix}[1]{P({#1})}
\newcommand{\projectedmatrixi}[2]{P_{#1}({#2})}
%\newcommand{\oGtilde}{{\oG^\prime}}
\newcommand{\oGtilde}{{\tilde\oG}}
\newcommand{\oGiprime}[1]{{\oGtilde_{#1}}}
\newcommand{\Dblock}[2]{\Delta_{{#1}{#2}}}
\newcommand{\Projection}[2]{\Pi_{#1} ({#2}) }
\newcommand{\ProjectionT}[3]{\Pi_{#1}^{#2} ({#3}) }
\newcommand{\lambdaregion}{$\lambdaset$-region}
\newcommand{\lambdaregions}{{\lambdaregion}s }


\newcommand{\make}[2]{{#2}_{#1}}
\newcommand{\indexa}{a}
\newcommand{\indexb}{b}
\newcommand{\indexdelta}{\Delta}
\newcommand{\lambdasetlambdaa}{\make{\indexa}{\lambdaset}}
\newcommand{\lambdasetlambdab}{\make{\indexb}{\lambdaset}}
\newcommand{\lamba}{\make{\indexa}{\llamb}}
\newcommand{\lambb}{\make{\indexb}{\llamb}}
\newcommand{\Acmatrixa}{\make{\indexa}{\Acmatrix}}
\newcommand{\Acmatrixb}{\make{\indexb}{\Acmatrix}}
\newcommand{\Acmatrixdelta}{\make{\indexdelta}{\Acmatrix}}
%\newcommand{\dira}{\make{\indexa}{\mu}}
%\newcommand{\dirb}{\make{\indexb}{\mu}}
\newcommand{\deriva}{\make{\indexa}{d}}
\newcommand{\derivb}{\make{\indexb}{d}}
\newcommand{\lipschitzfunction}{L}
\newcommand{\lipschitz}[1]{\lipschitzfunction({#1})}
\newcommand{\crossing}[1]{\lambdatwo^{({#1})}}
\newcommand{\nbcrossing}[0]{q}
%\newcommand{\crossingset}[1]{\lambdaset^{#1}}
\newcommand{\Region}{\Phi}
\newcommand{\region}{\phi}
\newcommand{\regioni}[1]{\region^{({#1})}}






%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mapxk}[1]{\mapx^{#1}}
\newcommand{\mapxi}[1]{\mapx_{#1}}
\newcommand{\mapXi}[1]{\mapX_{#1}}
\newcommand{\mapxki}[2]{\mapxk{#1}_{#2}}
\newcommand{\mapxconv}{x^\star}



\newcommand{\norm}[1]{\| {#1} \|}
\newcommand{\Norm}[1]{\left\| {#1} \right\|}
\newcommand{\singlenorm}[1]{| {#1} |}
\newcommand{\Singlenorm}[1]{\left| {#1} \right|}
\newcommand{\blocknorm}[1]{\norm{#1}}
\newcommand{\specialnorm}[2]{\norm{#1}_{#2}}
\newcommand{\Specialnorm}[2]{\Norm{#1}_{#2}}
\newcommand{\hatmapping}{\hat\mapping}
\newcommand{\mappingcompo}{\circ}
\newcommand{\modulus}{\alpha}
%
\newcommand{\mappingx}[1]{\mapping({#1})}
\newcommand{\mappingi}[1]{\mapping_{#1}}
\newcommand{\mappingix}[2]{\mappingi{#1}({#2})}
\newcommand{\hatmappingi}[1]{\hatmapping_{#1}}
\newcommand{\hatmappingix}[2]{\hatmappingi{#1}({#2})}
\newcommand{\Smappingx}[1]{\Smapping({#1})}
\newcommand{\Smappingi}[1]{\Smapping_{#1}}
\newcommand{\Smappingix}[2]{\Smappingi{#1}({#2})}
\newcommand{\mappingk}[1]{\mapping^{#1}}
\newcommand{\mappingki}[2]{\mappingk{#1}_{#2}}
\newcommand{\mappingkx}[2]{\mappingk{#1}({#2})}
\newcommand{\mappingkix}[3]{\mappingki{#1}{#2}({#3})}
\newcommand{\hatmappingk}[1]{\hatmapping^{#1}}
\newcommand{\hatmappingki}[2]{\hatmappingk{#1}_{#2}}
\newcommand{\hatmappingkix}[3]{\hatmappingki{#1}{#2}({#3})}
\newcommand{\Smappingk}[1]{\Smapping^{#1}}
\newcommand{\Smappingki}[2]{\Smappingk{#1}_{#2}}
\newcommand{\Smappingkx}[2]{\Smappingk{#1}({#2})}
\newcommand{\Smappingkix}[3]{\Smappingki{#1}{#2}({#3})}
\newcommand{\Amappingk}[1]{\Amapping^{#1}}
\newcommand{\Amappingki}[2]{\Amappingk{#1}_{#2}}
\newcommand{\Amappingkx}[2]{\Amappingk{#1}({#2})}
\newcommand{\Amappingkix}[3]{\Amappingki{#1}{#2}({#3})}
\newcommand{\alphamappingi}[1]{\alphamapping_{#1}}
\newcommand{\alphamappingx}[1]{\alphamapping({#1})}
\newcommand{\alphamappingix}[2]{\alphamappingi{#1}({#2})}
%
\newcommand{\newtonmappingi}[1]{\newtonmapping_{#1}}
\newcommand{\newtonmappingx}[1]{\newtonmapping({#1})}
\newcommand{\newtonmappingix}[2]{\newtonmappingi{#1}({#2})}
%
\newcommand{\newtonSmapping}{\check{\Smapping}}
\newcommand{\unitSmapping}{\dot{\Smapping}}
\newcommand{\GP}{GP}
\newcommand{\diagSmapping}{\ddot{\Smapping}}
\newcommand{\newtonAmapping}{\check{\Amapping}}
\newcommand{\diagAmapping}{\ddot{\Amapping}}
\newcommand{\newtonAmappingk}[1]{\newtonAmapping^{#1}}
\newcommand{\diagAmappingk}[1]{\diagAmapping^{#1}}
\newcommand{\CGP}{CGPML}
\newcommand{\SAA}{SAA}



\newcommand{\Ptk}[1]{r({#1})}
\newcommand{\Ptmax}{\bar r}
\newcommand{\Pseq}{\rho}
\newcommand{\Pseqk}[1]{\Pseq^{#1}}
\newcommand{\Pseqkj}[2]{\Pseq^{#1}\!({#2})}


%%%%%%%%%%%%%%%%%%%%


\newcommand{\edgefunction}{\epsilon}
\newcommand{\edge}[1]{\edgefunction({#1})}
\newcommand{\edgei}[2]{\edgefunction_{#1}({#2})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\nonviolatingsymbol}{\bar \violatingsymbol}
\newcommand{\nonviolatingsetsymbol}{\bar \violatingsetsymbol}
%%%% change this
\newcommand{\setviolating}[1]{\violatingsetsymbol_{#1}}
\newcommand{\setnonviolating}[1]{\nonviolatingsetsymbol_{#1}}
\newcommand{\matrixviolating}[1]{\violatingsymbol_{#1}}
\newcommand{\matrixnonviolating}[1]{\nonviolatingsymbol_{#1}}
% 
\newcommand{\setviolatingi}[1]{\violatingsetsymbol_{#1}}
\newcommand{\setnonviolatingi}[1]{\nonviolatingsetsymbol_{#1}}
\newcommand{\setviolatingx}[1]{\violatingsetsymbol({#1})}
\newcommand{\setnonviolatingx}[1]{\nonviolatingsetsymbol({#1})}
\newcommand{\setviolatingix}[2]{\setviolatingi{#1}({#2})}
\newcommand{\setnonviolatingix}[2]{\setnonviolatingi{#1}({#2})}
\newcommand{\setviolatingspecial}{\hat{\violatingsetsymbol}}
\newcommand{\unitvector}[1]{e^{#1}}
\newcommand{\unitvectori}[1]{e_{#1}}
\newcommand{\matrixviolatingx}[1]{\violatingsymbol({#1})}
\newcommand{\matrixnonviolatingx}[1]{\nonviolatingsymbol({#1})}
\newcommand{\matrixviolatingi}[1]{\violatingsymbol_{#1}}
\newcommand{\matrixnonviolatingi}[1]{\nonviolatingsymbol_{#1}}
\newcommand{\matrixviolatingix}[2]{\matrixviolatingi{#1}({#2})}
\newcommand{\matrixnonviolatingix}[2]{\matrixnonviolatingi{#1}({#2})}
\newcommand{\matrixordering}[1]{\orderingsymbol_{#1}}
\newcommand{\llambproj}{\bar \llamb}
\newcommand{\identityi}[1]{\identitysymbol_{#1}}
\newcommand{\tildeidentitysymbol}{\tilde \identitysymbol}
\newcommand{\tildeidentityi}[1]{\tildeidentitysymbol_{#1}}
\newcommand{\tildematrixidentitysymbol}{\tilde \matrixidentitysymbol}
%\newcommand{\tildematrixidentityi}[1]{\tildematrixidentitysymbol({#1})}
\newcommand{\tildematrixidentityi}[1]{\tildematrixidentitysymbol_{#1}}


\newcommand{\cst}{c}
\newcommand{\Cst}{C}
\newcommand{\Csti}[1]{\Cst_{#1}}
\newcommand{\cstn}{r}
\newcommand{\cstni}[1]{\cstn_{#1}}
\newcommand{\cstM}{M}
\newcommand{\cstMbis}{\bar \cstM}
\newcommand{\cstj}[1]{\cst_{#1}}
\newcommand{\cstx}[1]{\cst({#1})}
\newcommand{\cstjx}[2]{\cstj{#1}({#2})}
\newcommand{\nA}{\cstn}
\newcommand{\nAi}[1]{\nA_{#1}}
\newcommand{\CLcoef}{\alpha}
\newcommand{\CLcoefbis}{\hat \CLcoef}
\newcommand{\CLcoefter}{\bar \CLcoef}
\newcommand{\CLcoefj}[1]{\CLcoef_{#1}}
\newcommand{\CLcoefbisj}[1]{\CLcoefbis_{#1}}
\newcommand{\CLcoefterj}[1]{\CLcoefter_{#1}}
\newcommand{\GDfunction}{h}
\newcommand{\GDx}[1]{\GDfunction({#1})}
\newcommand{\GDxaT}[3]{\GDfunction({#1},{#2},{#3})}
\newcommand{\minimumdist}{\Delta}
\newcommand{\ballradius}{\delta}

\newcommand{\subderiv}{s}
\newcommand{\dgnom}{\gamma}
\newcommand{\dnom}{\alpha}
\newcommand{\snom}{\sigma}
\newcommand{\dgv}{\dgnom}
\newcommand{\dgnv}{\bar \dgnom}
\newcommand{\dv}{\dnom}
\newcommand{\dnv}{\bar \dnom}
\newcommand{\sv}{\snom}
\newcommand{\snv}{\bar \snom}


\newcommand{\mpneibi}[1]{\eta_{#1}}
\newcommand{\mpdimension}{d}
\newcommand{\mpxi}[1]{\mpdimension^{(\xx)}_{#1}}
\newcommand{\mplambi}[1]{\mpdimension^{(\llamb)}_{#1}}
\newcommand{\mpiter}[2]{\nu_{#1}({#2})}
\newcommand{\mpnumber}{l}
\newcommand{\mpbit}{b}

\newcommand{\genericn}{n}
\newcommand{\genericlambda}{\xi}
\newcommand{\genericdirection}{d}
\newcommand{\genericdirectioni}[1]{\genericdirection_{#1}}
\newcommand{\directionk}[1]{\genericdirection^{#1}}

\newcommand{\lambtilde}{\tilde\llamb}
\newcommand{\lambtildei}[1]{\lambtilde_{#1}}

%%%

\newcommand{\sequencet}[1]{\sequencesymbol^{#1}}
\newcommand{\sequenceti}[2]{\sequencet{#1}_{#2}}
\newcommand{\subsequenceseti}[1]{W_{#1}}



%%%%%%%%%%%%%


\newcommand{\boxletter}{b}
\newcommand{\boxl}{\textup{\b{$\boxletter$}}} 
\newcommand{\boxu}{\bar{\boxletter}}
\newcommand{\boxli}[1]{{\boxl}_{#1}} 
\newcommand{\boxui}[1]{{\boxu}_{#1}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\projectedllamb}{\tilde \llamb}
\newcommand{\projectedllambfni}[1]{\projectedllamb({#1})}
\newcommand{\projectedllambfnii}[2]{\projectedllambi{#2}({#1})}
\newcommand{\projectedllambi}[1]{\projectedllamb_{#1}}



%%%%%%%%%% CCCA

\newcommand{\hidden}[2]{#1}


\newcommand{\amplitude}{a}
\newcommand{\complexmessage}{m}
\newcommand{\bpmessage}{\tilde{\complexmessage}}
\newcommand{\complexnoise}{n}
\newcommand{\receipt}{r}
\newcommand{\complexgain}{h}
\newcommand{\amplitudei}[1]{\amplitude_{#1}}
\newcommand{\messagei}[1]{\complexmessage_{#1}}
\newcommand{\bpmessagei}[1]{\bpmessage_{#1}}
\newcommand{\receipti}[1]{{\receipt}_{#1}}
\newcommand{\noisei}[1]{{\complexnoise}_{#1}}
\newcommand{\hatreceipti}[1]{{\hat \receipt}_{#1}}
\newcommand{\gainij}[2]{\complexgain_{{#1}{#2}}}



\newcommand{\exposingle}{\text{s}}
\newcommand{\expomultiple}{\text{m}}
\newcommand{\Tset}{\Omega}
\newcommand{\Tsets}{\Tset^{\exposingle}}
\newcommand{\Tsetm}{\Tset^{\expomultiple}}
\newcommand{\sumtrans}[3]{\underset{\underset{\hspace{-3mm}{#2}\in{#3}\hspace{-3mm}}{{#1}:}}{\sum}}
\newcommand{\maxtrans}[3]{\underset{\underset{\hspace{-3mm}{#2}\in{#3}\hspace{-3mm}}{{#1}:}}{\max}}


%\newcommand{\decal}{\hspace{-2mm}}


\newcommand{\Glagrangian}{l}
\newcommand{\Gdual}{q}
\newcommand{\Gprimal}{f}
%\newcommand{\Lobjectivei}[1]{\Gobjective_{#1}}
\newcommand{\Llagrangiani}[1]{\Glagrangian_{#1}}
\newcommand{\Lduali}[1]{\Gdual_{#1}}
\newcommand{\Lprimali}[1]{\Gprimal_{#1}}


\newcommand{\Glambda}{\llamb}
\newcommand{\Gmu}{\mmu}

\newcommand{\dist}{\text{dist}}
\newcommand{\eunit}{u}




%%%%%%%%%%%%%%%%%%%%%%%%%  STOCHASTIC

\newcommand{\compact}{K}
\newcommand{\compacttwo}{\bar \compact}
\newcommand{\compacti}[1]{\compact_{#1}}
\newcommand{\stochF}[1]{\stochFfunction({#1})}
\newcommand{\stochFempfunction}{\hat \stochFfunction}
\newcommand{\stochFempkfunction}[1]{\stochFempfunction^{#1}}
\newcommand{\stochFempk}[3]{\stochFempkfunction{#1}({#2};{#3})}
\newcommand{\stochx}[1]{\stochxfunction({#1})}
\newcommand{\stochxxi}[2]{\stochxfunction_{#1}({#2})}
\newcommand{\stochX}[1]{\stochXfunction({#1})}
\newcommand{\stochXifunction}[1]{\stochXfunction_{#1}}
\newcommand{\stochXi}[2]{\stochXifunction{#1}({#2})}
\newcommand{\functionalXi}[1]{\functionalX_{#1}}
\newcommand{\stochobjectiveifunction}[1]{\stochobjectivefunction_{#1}}
\newcommand{\stochobjective}[2]{\stochobjectivefunction({#1},{#2})}
\newcommand{\stochobjectivei}[3]{\stochobjectiveifunction{#1}({#2},{#3})}
%\newcommand{\expectation}[1]{E \left\lbrack {#1} \right\rbrack }
%\newcommand{\smallexpectation}[1]{E \lbrack {#1} \rbrack }
\newcommand{\expectationsymbol}{E}%{\textup{E}}
\newcommand{\expectation}[1]{\expectationsymbol{}\left\lbrack {#1} \right\rbrack }
\newcommand{\smallexpectation}[1]{\expectationsymbol{}\lbrack {#1} \rbrack }
\newcommand{\stochRconstfunction}{\Rconst}
\newcommand{\stochRconst}[1]{\stochRconstfunction({#1})}
\newcommand{\stochcconstfunction}{\cconst}
\newcommand{\stochcconst}[1]{\stochcconstfunction({#1})}
\newcommand{\stochconstraintfunction}{\constraintfunction}
\newcommand{\stochconstraintineqfunction}{\constraintineqfunction}
\newcommand{\stochconstrainteqfunction}{\constrainteqfunction}
\newcommand{\stochconstraint}[2]{\constraintfunction({#1},{#2})}
\newcommand{\stochconstraintineq}[2]{\constraintineqfunction({#1},{#2})}
\newcommand{\stochconstrainteq}[2]{\constrainteqfunction({#1},{#2})}
\newcommand{\stochconstraintifunction}[1]{\stochconstraintfunction_{#1}}
\newcommand{\stochconstraintineqifunction}[1]{\stochconstraintineqfunction_{#1}}
\newcommand{\stochconstrainteqifunction}[1]{\stochconstrainteqfunction_{#1}}
\newcommand{\stochconstrainti}[3]{\constraintifunction{#1}({#2},{#3})}
\newcommand{\stochconstraintineqi}[3]{\constraintineqifunction{#1}({#2},{#3})}\newcommand{\stochconstrainteqi}[3]{\constrainteqifunction{#1}({#2},{#3})}
\newcommand{\stochlagrangian}[2]{\stochlagrangianfunction({#1},{#2})}
\newcommand{\stochlagrangianifunction}[1]{\stochlagrangianfunction_{#1}}
\newcommand{\stochlagrangiani}[3]{\stochlagrangianifunction{#1}({#2},{#3})}
\newcommand{\stochl}[3]{\stochlfunction({#1},{#2},{#3})}
\newcommand{\stochlifunction}[1]{\stochlfunction_{#1}}
\newcommand{\stochli}[4]{\stochlifunction{#1}({#2},{#3},{#4})}
\newcommand{\stochdual}[1]{\stochdualfunction({#1})}
\newcommand{\stochdualifunction}[1]{\stochdualfunction_{#1}}
\newcommand{\stochduali}[2]{\stochdualifunction{#1}({#2})}
\newcommand{\stochg}[2]{\stochgfunction({#1},{#2})}
\newcommand{\stochgifunction}[1]{\stochgfunction_{#1}}
\newcommand{\stochgi}[3]{\stochgifunction{#1}({#2},{#3})}
\newcommand{\stochLVij}[3]{\LVij{#1}{#2}({#3})} 
\newcommand{\stochLvi}[2]{\Lvi{#1}(#2)}
\newcommand{\stochLvix}[3]{\Lvi{#1}({#2},{#3})}
\newcommand{\stochconstraintlocalijfunction}[2]{\constraintlocalijfunction{#1}{#2}}
\newcommand{\stochconstraintlocalij}[4]{\stochconstraintlocalijfunction{#1}{#2}({#3},{#4})}
\newcommand{\stochconstraintineqlocalij}[4]{\constraintineqlocalijfunction{#1}{#2}({#3},{#4})}
\newcommand{\stochbvectori}[2]{\bvectori{#1}(#2)}
\newcommand{\stochxsolfunction}{\xsolfunction}
\newcommand{\stochxsol}[2]{\xsolfunction({#1},{#2})}
\newcommand{\stochxsolifunction}[1]{\stochxsolfunction_{#1}}
\newcommand{\stochxsoli}[3]{\xsolifunction{#1}({#2},{#3})}
\newcommand{\stochsetxsolifunction}[1]{\mathcal{X}_{#1}}
\newcommand{\stochsetxsoli}[3]{\stochsetxsolifunction{#1}({#2},{#3})}

\newcommand{\lambdak}[1]{\llamb^{#1}}
\newcommand{\lambdaki}[2]{\lambdak{#1}_{#2}}
\newcommand{\step}{a}
\newcommand{\stepk}[1]{\step^{#1}}
\newcommand{\magnitude}[1]{O({#1})}
\newcommand{\maxstochdualfunction}{\stochdualfunction^*}

\newcommand{\modelkfunction}[1]{\hat \dualfunction^{#1}}
\newcommand{\modelk}[3]{\modelkfunction{#1}({#2};{#3})}
\newcommand{\modelkifunction}[2]{\modelkfunction{#1}_{#2}}
\newcommand{\modelki}[4]{\modelkifunction{#1}{#2}({#3};{#4})}
\newcommand{\functionx}[1]{\function({#1})}
\newcommand{\functionk}[1]{\hat \function^{#1}}
\newcommand{\functionki}[2]{\functionk{#1}_{#2}}
\newcommand{\functionkx}[2]{\functionk{#1}({#2})}
\newcommand{\functionkix}[3]{\functionki{#1}{#2}({#3})}
\newcommand{\functionsol}{\function^\star}
\newcommand{\fkx}[2]{\functionk{#1} ({#2})}
\newcommand{\fkxi}[3]{\functionk{#1} _{#3} ({#2})}
\newcommand{\Descentkfunction}[1]{p^{#1}}
\newcommand{\Descentk}[5]{\Descentkfunction{#1}({#2},{#4},{#5};{#3})}
\newcommand{\Descentki}[6]{\Descentkfunction{#1}_{#6}({#2},{#4},{#5};{#3})}
\newcommand{\descentkfunction}[1]{\pi^{#1}}
\newcommand{\descentk}[5]{\descentkfunction{#1}({#2},{#3},{#5};{#4})}

\newcommand{\stochdeltadual}[1]{\Delta_{\modelkfunction{#1}}}
\newcommand{\stochdualzero}[1]{\Sigma_{\modelkfunction{#1}}}
%\newcommand{\stochxsolkfunction}[1]{{x^{#1}}^*}
%\newcommand{\stochxsolk}[2]{\stochxsolkfunction{#1}(#2)}
%\newcommand{\stochxsolkifunction}[2]{{x^{#1}_{#2}}^*}
%\newcommand{\stochxsolki}[3]{\stochxsolkifunction{#1}{#2}(#3)}
\newcommand{\stochxsolkfunction}[1]{\hat \stochxfunction^{#1}}
\newcommand{\stochxsolk}[2]{\stochxsolkfunction{#1}(#2)}
\newcommand{\stochxsolkifunction}[2]{\stochxsolkfunction{#1}_{#2}}
\newcommand{\stochxsolki}[3]{\stochxsolkifunction{#1}{#2}(#3)}


%



\newcommand{\dimx}{\NN}
\newcommand{\dimlambda}{M}

\newcommand{\xxk}[1]{\xx^{#1}}
\newcommand{\xxki}[2]{\xx^{#1}_{#2}}
\newcommand{\xxka}[2]{\xxk{#1} ({#2})}
\newcommand{\xxkai}[3]{\xxki{#1}{#3} ({#2})}
\newcommand{\zzk}[1]{\zz^{#1}}
\newcommand{\zzki}[2]{\zz^{#1}_{#2}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cosinus}[1]{\textup{cos}(#1)}

\newcommand{\coshconst}{\gamma}


\newcommand{\constraint}[1]{\constraintfunction({#1})}
\newcommand{\constraintifunction}[1]{\constraintfunction_{#1}}
\newcommand{\constrainti}[2]{\constraintifunction{#1}({#2})}
\newcommand{\constraintikfunction}[2]{\constraintifunction{#1,#2}}
\newcommand{\constraintik}[3]{\constraintikfunction{#1}{#2}({#3})}

\newcommand{\constrainteqfunction}{\constraintfunction^{\text{e}}}
\newcommand{\constrainteq}[1]{\constrainteqfunction({#1})}
\newcommand{\constrainteqifunction}[1]{\constrainteqfunction_{#1}}
\newcommand{\constrainteqi}[2]{\constrainteqifunction{#1}({#2})}
\newcommand{\constraintineqfunction}{\constraintfunction^{\text{i}}}
\newcommand{\constraintineq}[1]{\constraintineqfunction({#1})}
\newcommand{\constraintineqifunction}[1]{\constraintineqfunction_{#1}}
\newcommand{\constraintineqi}[2]{\constraintineqifunction{#1}({#2})}
\newcommand{\constraintineqlocalijfunction}[2]{\constraintlocalijfunction{#1}{#2}^{\text{i}}}
\newcommand{\constraintineqlocalij}[3]{\constraintineqlocalijfunction{#1}{#2}({#3})}
\newcommand{\constraintlocalij}[3]{\constraintlocalijfunction{#1}{#2}({#3})}
\newcommand{\constraintlocalijkfunction}[3]{(\constraintlocalijfunction{#1}{#2})_{#3}}
\newcommand{\constraintlocalijk}[4]{\constraintlocalijkfunction{#1}{#2}{#3}({#4})}
\newcommand{\constraintineqlocalconsti}[1]{\constraintineqlocalconst_{#1}}


\newcommand{\cconstx}[1]{\cconst ({#1})}
\newcommand{\Lvix}[2]{\Lvi{#1}({#2})}
\newcommand{\Lvikfunction}[2]{\Lvi{#1,#2}}
\newcommand{\llambik}[2]{\llambi{#1,#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\deltalambi}[1]{\deltalamb_{#1}}
\newcommand{\freexxi}[1]{ \freexx_{#1}}
\newcommand{\freexsolfunction}{\freexx^*}
\newcommand{\freexsolifunction}[1]{\freexsolfunction_{#1}}
\newcommand{\freexsol}[2]{\freexsolfunction({#2};{#1})}
\newcommand{\freexsoli}[3]{\freexsolfunction_{#1}({#3};{#2}) }
\newcommand{\freelagrangianfunction}{ \tilde l}
\newcommand{\freelagrangianifunction}[1]{ \freelagrangianfunction_{#1}}
\newcommand{\freelagrangianarg}[3]{({#1},{#3};{#2})}
\newcommand{\freelagrangiani}[4]{ \freelagrangianifunction{#1}\freelagrangianarg{#2}{#3}{#4}}
\newcommand{\freegrad}{\tilde \delta }
\newcommand{\freegradi}[1]{\freegrad_{#1} }
\newcommand{\freespace}[1]{Y({#1})}
\newcommand{\kron}[2]{\delta_{{#1}{#2}}}


\newcommand{\negativeform}{h}
\newcommand{\negativeformi}[1]{\negativeform_{#1}}
\newcommand{\negativeformix}[2]{\negativeform_{#1}({#2})}


%%%%%%%%%%%%%

\newcommand{\convexcave}[2]{#2}

\newcommand{\smallequal}{ \hspace{-2mm}=\hspace{-2mm}}


\newcommand{\minsdfunction}{\tilde s}
\newcommand{\minsd}[1]{\minsdfunction{#1}}


%%%%


\newcommand{\maphatGfunction}{\hat{\mapGfunction}}
\newcommand{\maphatGi}[1]{\maphatGfunction_{#1}}
\newcommand{\maphatGifx}[3]{\maphatGi{#1}({#2},{#3})}
\newcommand{\mapfx}[2]{\mapfunction({#1},{#2})}
\newcommand{\mapGfx}[2]{\mapGfunction({#1},{#2})}
\newcommand{\mapGi}[1]{\mapGfunction_{#1}}
\newcommand{\mapGifx}[3]{\mapGi{#1}({#2},{#3})}
\newcommand{\mapSfx}[2]{\mapSfunction({#1},{#2})}
\newcommand{\mapAfx}[2]{\mapAfunction({#1},{#2})}
\newcommand{\mapAi}[1]{\mapAfunction_{#1}}
\newcommand{\mapAifx}[3]{\mapAi{#1}({#2},{#3})}
\newcommand{\mapOfx}[2]{\mapOfunction({#1},{#2})}
\newcommand{\mapGGfx}[2]{\mapGGfunction({#1},{#2})}
\newcommand{\functionh}{h}
\newcommand{\functionhx}[1]{\functionh({#1})}


%%%%%%%%%%%%%%ù

\newcommand{\maxd}{d}

\newcommand{\notFx}[1]{\notF({#1})}

\newcommand{\rooffunction}{h}
\newcommand{\roofk}[1]{\rooffunction^{#1}}

\newcommand{\Zrho}{\rho}
\newcommand{\Zrhok}[1]{\Zrho^{#1}}
\newcommand{\Ztheta}{\theta}
\newcommand{\Zthetak}[1]{\Ztheta^{#1}}
\newcommand{\Zrhoone}{\Zrho_1}
\newcommand{\Zrhotwo}{\Zrho_2}
\newcommand{\Zrhoprime}{\phi}
\newcommand{\Zeps}{\epsilon}
\newcommand{\Zrhomax}{\bar \Zrho}
\newcommand{\ZrhomaxZrho}[1]{\Zrhomax({#1})}
%\newcommand{\ZZ}{Z}
\newcommand{\ZZ}{A}
\newcommand{\ZX}[1]{\ZZ^{#1}}
\newcommand{\ZZrho}[1]{\ZZ({#1})}
\newcommand{\ZXZrho}[2]{\ZX{#1}({#2})}
\newcommand{\ZoutZ}{\ZZ}
\newcommand{\ZoutX}[1]{\ZoutZ^{#1}}
\newcommand{\ZoutZrho}[1]{\ZoutZ({#1})}
\newcommand{\ZoutXZrho}[2]{\ZoutX{#1}({#2})}
\newcommand{\ZinZ}{\bar\ZZ}
\newcommand{\ZinX}[1]{\ZinZ^{#1}}
\newcommand{\ZinZrho}[1]{\ZinZ({#1})}
\newcommand{\ZinXZrho}[2]{\ZinX{#1}({#2})}
\newcommand{\ZbarZrho}[1]{\hat \ZZ({#1})}
\newcommand{\sgradfunction}{S}
\newcommand{\sgradkfunction}[1]{\sgradfunction^{#1}}
\newcommand{\sgrad}[1]{\sgradfunction({#1})}
\newcommand{\sgradk}[2]{\sgradkfunction{#1}({#2})}
\newcommand{\sdi}[1]{\sd_{#1}}
\newcommand{\sdk}[1]{\sd^{#1}}
\newcommand{\sdki}[2]{\sdk{#1}_{#2}}
\newcommand{\sdix}[2]{\sdi{#1}({#2})}
\newcommand{\sdx}[1]{\sd({#1})}
\newcommand{\sdkx}[2]{\sdk{#1}({#2})}
\newcommand{\sdkix}[3]{\sdki{#1}{#2}({#3})}
\newcommand{\Zk}{\bar k}
\newcommand{\Zkother}{\hat k}
\newcommand{\Zkotherother}{\tilde k}
\newcommand{\Zkgen}{t}
\newcommand{\Zimpact}[1]{\hat k ({#1})}
\newcommand{\Zgamma}{\gamma}
\newcommand{\Zsgamma}{\psi}
\newcommand{\Zphi}{\phi}
\newcommand{\Zeta}{\eta}
\newcommand{\Zbeta}{\beta}
\newcommand{\Zalpha}{\alpha}
\newcommand{\Zalphanew}{\Zsgamma}
\newcommand{\Zd}{d}
\newcommand{\Zdrho}[1]{\Zd({#1})}
 \newcommand{\Zfunctionkx}[2]{\zeta^{#1}({#2})}
\newcommand{\Zsd}{s}
\newcommand{\Zsdx}[1]{\Zsd({#1})}
\newcommand{\Zsdk}[1]{\Zsd^{#1}}
\newcommand{\Zsdkx}[2]{\Zsdk{#1}({#2})}
\newcommand{\Zsdkxi}[3]{\Zsdk{#1}_{#3}({#2})}
\newcommand{\setofScales}{\mathcal{\Scale}}
\newcommand{\setofScalesi}[1]{\setofScales_{#1}}
\newcommand{\setofdiagScales}{\mathcal{\diagScale}}
\newcommand{\setofdiagScalesi}[1]{\setofdiagScales_{#1}}
\newcommand{\Zdelta}{\delta}
\newcommand{\Zdeltax}[1]{\Zdelta({#1})}
\newcommand{\ZdeltaC}[1]{\Zdelta_{#1}}
\newcommand{\ZdeltaCx}[2]{\ZdeltaC{#1}({#2})}

%\newcommand{\variaeps}{\epsilon}
\newcommand{\variafunction}{\delta}
\newcommand{\varia}[1]{\variafunction({#1})}

\newcommand{\llamblimit}{\tilde \llamb}
\newcommand{\mmulimit}{\tilde \mmu}
\newcommand{\divQ}{K}
\newcommand{\divQprime}{\bar \divQ}

%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\follows}{\sim}
\newcommand{\stocht}[1]{\stoch_{#1}}
\newcommand{\stochk}[1]{\stoch^{#1}}
\newcommand{\sample}{t}
\newcommand{\samples}{\bar \sample}
\newcommand{\samplesk}[1]{\samples({#1})}
\newcommand{\distrifunction}{F}
\newcommand{\distri}[1]{\distrifunction({#1})}
\newcommand{\distrifunctiontheta}[1]{\distrifunction_{#1}}
\newcommand{\distritheta}[2]{\distrifunctiontheta{#1}({#2})}
\newcommand{\distriGfunction}{G}
\newcommand{\distriG}[1]{\distriGfunction({#1})}
\newcommand{\distriGfunctiontheta}[1]{\distriGfunction_{#1}}
\newcommand{\distriGtheta}[2]{\distriGfunctiontheta{#1}({#2})}
\newcommand{\Fkfunction}[1]{\distrifunction^{#1}}
\newcommand{\Fk}[2]{\Fkfunction{#1}({#2})}
\newcommand{\distrifunctionk}[1]{\hat\distrifunction^{#1}}
\newcommand{\distrik}[2]{\distrifunctionk{#1}({#2})}
\newcommand{\thetaparam}{\theta}
\newcommand{\thetaparamk}[1]{\hat\thetaparam^{#1}}
\newcommand{\functionalZfunction}{Z}
\newcommand{\functionalZ}[1]{\functionalZfunction({#1})}


%%%

%\newcommand{\edge}{e}
\newcommand{\edgeij}[2]{({#1},{#2})}
\newcommand{\incidenceij}[2]{\incidence_{{#1}{#2}}}
\newcommand{\incidencei}[1]{\incidence_{{#1}}}
\newcommand{\incidenceistoch}[2]{\incidencei{#1}({#2})}
\newcommand{\incidenceijstoch}[3]{\incidenceij{#1}{#2}({#3})}
\newcommand{\bvectori}[1]{\bvector_{#1}}
\newcommand{\bvectoristoch}[2]{\bvectori{#1}({#2})}

%%%%%%%%%%%

\newcommand{\llambdest}{\bar \llamb}
\newcommand{\seg}{t}
\newcommand{\nseg}{\bar \seg }
\newcommand{\reducedspace}{\PROJsetoflambdas}



%%%%

\newcommand{\error}{e}
\newcommand{\errork}[1]{\error^{#1}}
\newcommand{\errori}[1]{\error_{#1}}
\newcommand{\errorki}[2]{\errork{#1}_{#2}}
\newcommand{\CAPhi}{\Phi}
\newcommand{\CAPhix}[1]{\CAPhi({#1})}
\newcommand{\CAPhii}[1]{\CAPhi_{#1}}
\newcommand{\CAPhiix}[2]{\CAPhii{#1}({#2})}

%%%%%%%%%%%%

\newcommand{\nesteA}{\mathcal{A}}
\newcommand{\nesteAa}[1]{\nesteA^{({#1})}}
\newcommand{\nestea}{\alpha}
\newcommand{\unitvec}{U}
\newcommand{\unitveci}[1]{\unitvec_{#1}}
\newcommand{\constantScale}{\hat \Scale}
\newcommand{\constantScalei}[1]{\constantScale_{#1}}

%%%

\newcommand{\kreach}{k^\star}
\newcommand{\kreachx}[1]{\kreach({#1})}

\newcommand{\generated}{t}
\newcommand{\gener}{s}


%%%%

\newcommand{\prprty}{p}
\newcommand{\prprtyx}[1]{\prprty({#1})}

%%%

\newcommand{\matrixleq}{\preceq}
\newcommand{\matrixgeq}{\succeq}
\newcommand{\matrixl}{\prec}
\newcommand{\matrixg}{\succ}

%%%%%

\newcommand{\dom}[1]{\text{\textup{dom}}({#1})}
\newcommand{\cone}[1]{\text{\textup{cone}}({#1})}
\newcommand{\notC}{C}
\newcommand{\polar}{*}   %




\newcommand{\setofallhalfspaces}{H}
\newcommand{\setofallactivehalfspaces}{\bar \setofallhalfspaces}
\newcommand{\soaahs}[1]{\setofallactivehalfspaces({#1})}
\newcommand{\setofhalfspaces}{A}
\newcommand{\setofactivehalfspaces}{\bar \setofhalfspaces}
\newcommand{\soahs}[1]{\setofactivehalfspaces({#1})}
\newcommand{\soahsk}[2]{\setofactivehalfspaces^{#1}({#2})}

%%%%

\newcommand{\degree}[1]{\textup{deg}({#1})}


\newcommand{\obj}{f_0}
\newcommand{\objx}[1]{\obj({#1})}
\newcommand{\ic}{f}
\newcommand{\ici}[1]{\ic_{#1}}
\newcommand{\icx}[1]{\ic({#1})}
\newcommand{\icix}[2]{\ici{#1}({#2})}
\newcommand{\ec}{h}
\newcommand{\eci}[1]{\ec_{#1}}
\newcommand{\ecx}[1]{\ec({#1})}
\newcommand{\ecix}[2]{\eci{#1}({#2})}
\newcommand{\objeps}{\tilde{f}_0}
\newcommand{\objepsxeps}[2]{\objeps({#1},{#2})}

\newcommand{\iy}{y}
\newcommand{\iyi}[1]{\iy_{#1}}
\newcommand{\ey}{z}
\newcommand{\eyi}[1]{\ey_{#1}}

\newcommand{\nic}{q}
\newcommand{\nec}{r}
\newcommand{\primalsol}{p^\star}
\newcommand{\dualsol}{d^\star}

\newcommand{\stationaryset}{\tilde \genericset}
\newcommand{\feasibleset}{\genericset}
\newcommand{\sideconstraintset}{S}
\newcommand{\sideconstraintseti}[1]{\sideconstraintset_{#1}}
\newcommand{\dualfeasibleset}{\genericsettwo}


\newcommand{\characteristicfunction}{\chi}
\newcommand{\characteristic}[1]{\characteristicfunction_{#1}}
\newcommand{\characteristicx}[2]{\characteristic{#1}({#2})}
\newcommand{\indicatorfunction}{1}
\newcommand{\indicator}[1]{\indicatorfunction_{#1}}
\newcommand{\indicatorx}[2]{\indicator{#1}({#2})}

%\renewcommand{\nn}{s}
%\renewcommand{\NN}{n}
\newcommand{\thnn}{s}
\newcommand{\thNN}{n}
\newcommand{\thNNi}[1]{\thNN_{#1}}

%%%%%%%%
\newcommand{\factorial}[1]{{#1}!}

%%

\newcommand{\Probafunction}{\textup{Pr}}
\newcommand{\Proba}[1]{\Probafunction\left({#1}\right)}
\newcommand{\proba}[1]{\Probafunction({#1})}
\newcommand{\Xnfunction}{\notx}%{X}
\newcommand{\Xn}[1]{\Xnfunction^{#1}}
\newcommand{\Xlimit}{\bar \notx}%{X}
\newcommand{\Xmu}{\Xlimit}%{\mu}
\newcommand{\barXn}[1]{\bar{\Xnfunction}^{#1}}
\newcommand{\notfn}[1]{\notf^{#1}}
\newcommand{\notfnx}[2]{\notfn{#1}({#2})}
%distri
%distrik
\newcommand{\stochnotf}{\tilde \notf}
\newcommand{\stochnotfxstoch}[2]{\stochnotf({#1},{#2})}


%%%%%%%%%%

\newcommand{\quasiD}{D}
\newcommand{\quasip}{p}
\newcommand{\quasiq}{q}
\newcommand{\quasixi}{\xi}
\newcommand{\quasitau}{\tau}
\newcommand{\quasinu}{\nu}
\newcommand{\quasiDk}[1]{{\quasiD^{#1}}}
\newcommand{\quasipk}[1]{{\quasip^{#1}}}
\newcommand{\quasiqk}[1]{{\quasiq^{#1}}}
\newcommand{\quasixik}[1]{{\quasixi^{#1}}}
\newcommand{\quasitauk}[1]{{\quasitau^{#1}}}
\newcommand{\quasinuk}[1]{{\quasinu^{#1}}}

%%%

\newcommand{\ipmu}{\mu}
\newcommand{\ipmuk}[1]{\ipmu^{#1}}
%\newcommand{\ipxmu}{\notx^{\ipmu}}
\newcommand{\ipxmu}[1]{\bar{\notx}({#1})}
\newcommand{\ipxsol}{\xxsol}
\newcommand{\ipysol}{\yy^\star}
\newcommand{\ipysoli}[1]{\ipysol_{#1}}
%\newcommand{\ipymu}{\yy^{\ipmu}}
%\newcommand{\ipymui}[1]{\ipymu_{#1}}
%\newcommand{\ipymux}[1]{\ipymu({#1})}
%\newcommand{\ipymuix}[2]{\ipymui{#1}({#2})}
\newcommand{\ipy}{\yy}
\newcommand{\ipymux}[2]{\ipy({#1},{#2})}
\newcommand{\ipymuix}[3]{\ipy_{#2}({#1},{#3})}
\newcommand{\ipf}{\obj} % \notf
\newcommand{\ipc}{\ic}  % c
\newcommand{\ipB}{b}
\newcommand{\ipfx}[1]{\ipf({#1})}
\newcommand{\ipcx}[1]{\ipc({#1})}
\newcommand{\ipci}[1]{\ipc_{#1}}
\newcommand{\ipcix}[2]{\ipci{#1}({#2})}
%\newcommand{\ipBxmu}[2]{\ipB({#1},{#2})}
\newcommand{\ipBmu}{\ipB^{\ipmu}}
\newcommand{\ipBxmu}[1]{\ipBmu({#1})}

\newcommand{\proxc}{c}
\newcommand{\proxck}[1]{\proxc^{#1}}
\newcommand{\proxL}{\bar{l}}
\newcommand{\proxLxyc}[3]{\proxL({#1},{#2},{#3})}
\newcommand{\proxpsy}{\psi}
\newcommand{\proxpsyxyc}[3]{\proxpsy({#1},{#2},{#3})}
\newcommand{\proxT}{T}
\newcommand{\proxTx}[1]{\proxT{#1}}
\newcommand{\proxP}{P}
\newcommand{\proxPx}[1]{\proxP{#1}}

\newcommand{\sqpd}{d}
\newcommand{\sqpdk}[1]{\sqpd^{#1}}
\newcommand{\sqpdx}{\sqpd_{\xx}}
\newcommand{\sqpdy}{\sqpd_{\yy}}
\newcommand{\sqpdz}{\sqpd_{\zz}}
\newcommand{\slack}{u}
\newcommand{\slacki}[1]{\slack_{#1}}
\newcommand{\hessianlagrangian}{H}
\newcommand{\hessianlagrangiank}[1]{\hessianlagrangian^{#1}}

%%%%%


\newcommand{\stochi}[1]{\stoch_{#1}}
\newcommand{\stochij}[2]{\stoch_{#1 #2}}
\newcommand{\flowstoch}[1]{\flow({#1})}
\newcommand{\flowi}[1]{\flow_{#1}}
\newcommand{\Flowstoch}[1]{\Flow({#1})}
\newcommand{\Flowistoch}[2]{\Flowi{#1}({#2})}
\newcommand{\flowistoch}[2]{\flowi{#1}({#2})}
\newcommand{\flowijstoch}[3]{\flowij{#1}{#2}({#3})}
\newcommand{\incidencestoch}[1]{\incidence({#1})}
\newcommand{\generistoch}[2]{\generi{#1}({#2})}
\newcommand{\generstoch}[1]{\gener({#1})}
\newcommand{\restrict}{B}
\newcommand{\restrictstoch}[1]{\restrict({#1})}
\newcommand{\restrictij}[2]{\restrict_{#1 #2}}
\newcommand{\restrictijstoch}[3]{\restrictij{#1}{#2}({#3})}


\newcommand{\flow}{x}
\newcommand{\Flow}{X}
\newcommand{\Flowi}[1]{\Flow_{#1}}
\newcommand{\flowij}[2]{\flow_{{#1}{#2}}}
\newcommand{\flowijk}[3]{\flow_{{#1}{#2}}}
\newcommand{\flowbis}{y}
\newcommand{\flowbisij}[2]{\flowbis_{{#1}{#2}}}
%\newcommand{\flowto}{\overrightarrow{\flow}}
\newcommand{\toback}[1]{\bar{\bar{#1}}}
\newcommand{\flowtoback}{\toback{\flow}}
\newcommand{\flowtobacki}[1]{\flowtoback_{#1}}
\newcommand{\flowtobackbis}{\toback{\flowbis}}
\newcommand{\flowto}{\vec{\flow}}
\newcommand{\flowtoij}[2]{\flowto_{{#1}{#2}}}
\newcommand{\flowtostoch}[1]{\flowto({#1})}
\newcommand{\flowtoijstoch}[3]{\flowtoij{#1}{#2}({#3})}
%\newcommand{\flowback}{\overleftarrow{\flow}}
%\newcommand{\flowback}{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{\flow}}}}}}
\newcommand{\flowback}{\reflectbox{{${\vec{\reflectbox{{${\flow}$}}}}$}}}
\newcommand{\flowbacktiny}{\reflectbox{\tiny{${\vec{\reflectbox{\tiny{${\flow}$}}}}$}}}
\newcommand{\flowbackij}[2]{\flowback_{{#1}{#2}}}
\newcommand{\flowbackstoch}[1]{\flowback({#1})}
\newcommand{\flowbackijstoch}[3]{\flowbackij{#1}{#2}({#3})}
\newcommand{\flowr}[1]{\flow^{#1}}
\newcommand{\flowrij}[3]{\flowr{#1}_{{#2}{#3}}}
\newcommand{\cmmdty}{k}
\newcommand{\cmmdtymax}{\bar\cmmdty}
\newcommand{\generi}[1]{\gener_{{#1}}}
\newcommand{\generr}[1]{\gener^{{#1}}}
\newcommand{\generri}[2]{\generr{#1}_{{#2}}}
\newcommand{\pwr}{p}
\newcommand{\pwri}[1]{\pwr_{#1}}
\newcommand{\pwrx}[1]{\pwr({#1})}
\newcommand{\pwrix}[2]{\pwri{#1}({#2})}
\newcommand{\pwrmax}{\bar{\pwr}}
\newcommand{\pwrmaxstoch}[1]{\pwrmax({#1})}
\newcommand{\pwrmaxi}[1]{\pwrmax_{#1}}
\newcommand{\pwrmaxistoch}[2]{\pwrmaxi{#1}({#2})}
\newcommand{\meannrg}{\bar e}
\newcommand{\meanpwr}{\meannrg}
\newcommand{\meantpwr}{\meannrg^{\textup{t}}}
%\newcommand{\meantpwrij}[2]{\meantpwr_{{#1}{#2}}}
\newcommand{\meantpwrij}[2]{\meanpwr^{#1}_{{#1}{#2}}}
\newcommand{\meanrpwr}{\meannrg^{\textup{r}}}
%\newcommand{\meanrpwrij}[2]{\meanrpwr_{{#1}{#2}}}
\newcommand{\meanrpwrij}[2]{\meanpwr^{#2}_{{#1}{#2}}}
\newcommand{\stochpwr}{e}
\newcommand{\stochtpwrij}[3]{\meantpwrij{#1}{#2}(\stoch)}
\newcommand{\stochrpwrij}[3]{\meanrpwrij{#1}{#2}(\stoch)}
\renewcommand{\Tnet}{t^{\textup{\tiny{net}}}}
\newcommand{\Tnetx}[1]{\Tnet({#1})}
\newcommand{\iTnet}{q}
\newcommand{\iTnetx}[1]{\iTnet({#1})}
\newcommand{\iTneti}[1]{\iTnet_{#1}}
\newcommand{\iTnetbis}{\breve{\flowbis}}
\newcommand{\supply}{b}
\newcommand{\supplyi}[1]{\supply_{#1}}
\newcommand{\capa}{\bar \flow}
\newcommand{\capastoch}[1]{\capa({#1})}
\newcommand{\capai}[1]{\capa_{#1}}
\newcommand{\capaij}[2]{\capa_{{#1}{#2}}}
%\newcommand{\capabis}{\bar \flowbis}
\newcommand{\capabis}{\bar \flow}
\newcommand{\capabisij}[2]{\capabis_{{#1}{#2}}}
\newcommand{\cardinality}[1]{\singlenorm{#1}}


\newcommand{\flowsr}{\dot{\flow}}
\newcommand{\setofsredges}{\setofedges^{\textup{s}}}
\newcommand{\flowsrijk}[3]{\flowsr_{#2 #1 #3}}
\newcommand{\setofbfedges}{\setofedges^{\textup{b}}}
\newcommand{\setofrelays}[2]{r({#1},{#2})}



\newcommand{\flowbf}{\mathring{\flow}}
\newcommand{\flowbfij}[2]{\flowbf_{#1 #2}}


\newcommand{\nbrelays}{q}
\newcommand{\SNRmin}{\SNR^{\min{}}}
\newcommand{\SNRmini}[1]{\SNRmin_{#1}}
\newcommand{\Pnoise}{P^{\complexnoise}}



\newcommand{\ethres}{\textup{\b{$e$}}}
\newcommand{\ethresi}[1]{\ethres_{#1}}


%%%%%%%%%%%%%%%
\newcommand{\fcarrier}{f}

\newcommand{\Real}[1]{\textup{Re} \lbrack {#1}\rbrack }
\newcommand{\Imaginary}[1]{\textup{Im}\[{#1}\]}

%%%

\newcommand{\ik}[1]{i^{#1}} %{i({#1})}
%
\newcommand{\MHz}{\textup{MHz}}
\newcommand{\GHz}{\textup{MHz}}

\newcommand{\obsolete}[1]{}
